Sparser Abelian High Dimensional Expanders

We present two new explicit constructions of Cayley high dimensional expanders (HDXs) over the abelian group $\mathbb{F}_2^n$. Our expansion proofs use only linear algebra and combinatorial arguments. The first construction gives local spectral HDXs of any constant dimension and subpolynomial degree $\exp(n^\epsilon)$ for every $\epsilon >0$, improving on a construction by Golowich [Gol23] which achieves $\epsilon =1/2$. [Gol23] derives these HDXs by sparsifying the complete Grassmann poset of subspaces. The novelty in our construction is the ability to sparsify any expanding Grassmannian posets, leading to iterated sparsification and much smaller degrees. The sparse Grassmannian (which is of independent interest in the theory of HDXs) serves as the generating set of the Cayley graph. Our second construction gives a 2-dimensional HDXs of any polynomial degree $\exp(\epsilon n$) for any constant $\epsilon > 0$, which is simultaneously a spectral expander and a coboundary expander. To the best of our knowledge, this is the first such non-trivial construction. We name it the Johnson complex, as it is derived from the classical Johnson scheme, whose vertices serve as the generating set of this Cayley graph. This construction may be viewed as a derandomization of the recent random geometric complexes of [LMSY23]. Establishing coboundary expansion through Gromov's "cone method" and the associated isoperimetric inequalities is the most intricate aspect of this construction. While these two constructions are quite different, we show that they both share a common structure, resembling the intersection patterns of vectors in the Hadamard code. We propose a general framework of such "Hadamard-like" constructions in the hope that it will yield new HDXs.

==> Yotam_s_drafts/alternative_construction.tex <==
\begin{definition}[Sparsified linear spherical building]
    Let \(\Y\) be a \(d\)-dimensional \(\lambda\)-expanding Grassmann poset. Let \(D = \set{d_0<d_1<\dots <d_{k-1}} \subseteq \set{0,1,\dots,d}\) be a set of \(k+1\) integers. The \(k\)-partite complex \(X_{\Y,D}^{lin}\) is the following. The vertices in the \(i\)-th part are all the \(W \in Y(d_i)\)\footnote{We emphasize that this includes \(\Y(0)\) in which case this is just a single point.}. The faces in \(X_{\Y,D}(i)\) are all  \(\set{W_0,W_1,\dots W_i}\) such that (there exists an ordering where) \(W_0 \subseteq W_1 \subseteq \dots \subseteq W_i\).
\end{definition}

\begin{definition}[Sparsified spherical building]
    Let \(\Y\) be a \(d\)-dimensional \(\lambda\)-expanding Grassmann poset. Let \(D = \set{d_0<d_1<\dots <d_k} \subseteq \set{0,1,\dots,d}\) be a set of \(k+1\) integers. The \((k+1)\)-partite complex \(X_{\Y,D}\) is the following. The vertices in the \(i\)-th part are all the \(x + W\) for \(x \in \F_2^{n}\) and \(W \in Y(d_i)\)\footnote{We emphasize that this includes \(\Y(0)\) in which case this is just \(\F_2^n\).}. The faces in \(X_{\Y,D}(i)\) are all  \(\set{x_0+W_0,x_1+W_1,\dots x_i +W_i}\) such that (there exists an ordering where) \(x_0+W_0 \subseteq x_1 + W_1 \subseteq \dots \subseteq x_i + W_i\).
\end{definition}

For the rest of this section we fix \(\Y\) and \(D\), and we denote by \(X[i] \subseteq X(0)\) the \(i\)-th part in this complex. We observe that the number of vertices in \(X[i]\) is \[\abs{X[i] } = 2^{n-d_i}\abs{\Y(i)}.\]
In addition, note that for every \(v=x+W_i \in X[i]\), its link is the following. The vertices are:
\begin{enumerate}
    \item \(x+W_t\) such that \(W_t \subseteq W_i\) and \(\dim(W_t) \in \sett{d \in D}{d < d_i}\).
    \item All \(x+W_t\) such that \(W_t \in \Y_{W_i}\) and \(\dim(W_t) \in \sett{d \in D}{d > d_i}\).
\end{enumerate}

\begin{enumerate}
    \item 
\end{enumerate}

==> Yotam_s_drafts/old/abstract.tex <==
We present two new explicit constructions of high dimensional Cayley expanders (HDX) over $\F_2^n$.

The first construction gives HDX of any constant dimension and subpolynomial degree $exp(n^\epsilon )$ for every $\epsilon >0$, improving on  Golowich'  construction [Gol23]  which achieves $\epsilon = \frac12$. We use and expand on [Gol23] idea on deriving HDX from a Grassmann poset which is sparsified from the complete Grassmaniann. The novelty in our construction is the ability to sparsify appropriate expanding Grassmannian posets, leading to iterated sparsification and smaller degrees. We note that this is still far from the best lower bound, $\Omega(n)$, on the degree of any expanding Cayley complex (or even Cayley graph) on $\F_2^n$.

Our second construction gives a 2-dimensional HDX of polynomial degree $\epsilon n$ for any constant $\epsilon >0$, which is simultaneously a spectral expander and a coboundary expander. To the best of our knowledge, this is the first such construction.We name it the {\em Johnson complex}, as it derives form the classical Johnson graph, which serves as its generating set. Thus, strong spectral expansion of is quite easy to obtain directly from the theory of association schemes. Coboundary expansion on the other hand is more subtle, and requires the development of new ideas for proving the isoperimetric inequalities necessary for implementing Gromov's {\em cone method}.

==> Yotam_s_drafts/old/complete-part-analysis.tex <==
In the following subsection, our goal is to prove that the subposet graph and subposet link graphs are expanders.

Let us begin with the case where \(i=0\).
\begin{claim} \label{claim:subposet-graph-no-intersection}
    Let \(m_2 > 2r\). Then \(\lambda(G_{0,r,m_2}) \leq r2^{2r-m_2+2}\).
\end{claim}

\begin{proof}
    We intend to use \pref{claim:close-distance}, comparing our adjacency operator to that of the complete graph \(J\) (with self loops). Its second largest eigenvalue is \(0\). Thus we must show the adjacency operator of our graph is \(4r2^{2r-m_2}\)-close to the complete graph, i.e. that for every matrix \(M\).
    \[\norm{A_M - J_M}_1 \leq 4r2^{2r-m_2}.\]
    Observe that \(J_M\) is the uniform distribution. Thus it is enough to show that
    \[p = \Prob[M' \sim J]{M' \not\sim M} \leq 2r2^{2r-m_2}\]
    where \(M'\) is sampled uniformly but the event is the neighbor event of \(M,M'\).
    Since this implies that 
    \[\norm{A_M - J_M}_1 = \sum_{M' \sim M} \frac{1}{deg(M)}- \frac{1}{|V|} + \sum_{M' \not\sim M}\frac{1}{|V|} = 1-(1-2p)=2p.\]
    We observe that if \(\row(M'), \row(M)\) and \(\col(M),\col(M')\) intersect trivially then they are neighbors. 
    % This is because the rank of \(M+M'\) is dimension of the image. Write \(M=\sum_{i=1}^r e_i \otimes f_i\) and \(M' = \sum_{i=1}^r g_i \otimes h_i\). Then we can find vectors \(v_1,v_2,\dots,v_r,u_1,u_2,\dots,u_r\) with \((M+M')v_i=f_i, (M+M')u_i=h_i\) where \(v_i\) is not orthogonal to \(e_i\) but orthogonal to all other row vectors. as \(\set{f_i} \cup \set{h_i}\) are independent indeed their rank is \(2r\) as required.
    Let us bound the probability that \(\row(M')\) has an intersection with a given subspace of dimension \(r\) (the same calculation shall hold for \(\col(M)\)). As \(\row(M')\) is a uniformly chosen subspace of dimension \(r\) inside \(\mathbb{F}_2^{m_2}\). Sampling a uniform random \(r\)-dimensional subspace is the same as sampling \(v_1 \ne 0\), \(v_2 \notin \span(v_1)\), \(v_3 \notin \span(v_1,v_2\),..., \(v_r \notin \span(v_1,v_2,\dots,v_{r-1})\). Thus
    \begin{align*}
        \prob{\row(M) \cap \row(M') \ne \set{0}} &= \prob{\dim(\row(M) + \row(M')) < 2r} \\
        &\geq \sum_{i=1}^r \cProb{}{v_i \in \row(M) + \span(v_1,\dots,v_{i-1})}{v_i \notin \span(v_1,\dots,v_{i-1})} \\
        &= \sum_{i=1}^r \frac{\prob{v_i \in \row(M) + \span(v_1,\dots,v_{i-1})}}{\prob{v_i \notin \span(v_1,\dots,v_{i-1})}}.
    \end{align*}
    Fixing \(i \leq r\) and \(v_1,v_2,\dots,v_{i_1}\), the probability that \(v_i \notin \span(v_1,v_2,\dots,v_{i-1})\) is at least \(1-2^{i-1-m_2} \geq \frac{1}{2}\) since \(i-1-m_2<r-m_2-1<-1\). Similarly, the probability that \(v_i \in \row(M) + \span(v_1,\dots,v_{i-1})\) is at most \(2^{d-m_2}\) where \(d\) is the dimension of the sum of spaces. This is at most \(2^{2r-m_2}\). Thus \(\prob{\row(M) \cap \row(M') \ne \set{0}} \leq r2^{2r-m_2+1}\) and the upper bound is proven. Union bounding this with the same upper bound for the \(\col\) spaces given the required bound.
\end{proof}

Before we continue to other cases, we need the following claim
\begin{claim} \label{claim:containment-graph-expansion}
    Let \(M\) be a rank \(m\) matrix. Let \(i \leq r\leq m\) such that \(i \leq \frac{r}{2}\) and \(m\geq 2r\). Let \(G=(L,R,E)\) be a bipartite graph between
    \[L = \sett{A \leq M}{rank(A) = r}\]
    and 
    \[R = \sett{B \leq M}{rank(B) = i}\]
    whose edges are \(E = \sett{(A,B)}{B \leq A}\). Then \(G\) is a \(10\sqrt{r} 2^{-\frac{r}{6}}\)-bipartite expander.
\end{claim}

\begin{proof}
    Let us first prove the theorem under the assumption that \(i \leq \frac{r}{3}\). It suffices to show that \(2\)-step walk from \(i\)-rank matrices to themselves is a \(\frac{r}{3}2^{-\frac{r}{3}+3}\)-two sided spectral expander. 

    Let \((M_0,M_2)\) be such that \(M_2\) is sampled by taking \(2\) steps from \(M\). Let us calculate the probability that the \(\row(M_0)\) and \(\row(M_2)\) intersect trivially. Let \(M_1\) be the middle vertex in the walk from \(M_0\) to \(M_2\). We note that \(\row(M_2)\) and \(\col(M_2)\) are uniform subspaces of \(\row(M_1)\) and \(\col(M_1)\) respectively. Hence this is the probability that a random \(i\)-subspace intersects with another (fixed) subspace. This probability is at most \(2i2^{2i-r}\) as in the proof of \pref{claim:subposet-graph-no-intersection}. Let \(P'\) be the random walk that goes from \(M_0\) to \(M_2\) if they have trivially intersecting rowspan and colspan. This random walk is the adjacency operator of \(G_{m,i,0}\). By \pref{claim:close-distance} we have that our graph has expansion \(\lambda(P') + 4i2^{2i-r}\). By \pref{claim:subposet-graph-no-intersection} \(\lambda(P') \leq i2^{2i-m+2})\). To sum up this case, we have that when \(i \leq \frac{r}{4}\), the second largest eigenvalue is bounded by \(\frac{r}{3}2^{-\frac{r}{3}+3}\).

    Now we do the general case, i.e. we assume that \(i \geq \frac{r}{3}\) and localize via \pref{lem:local-to-global}.
    %
    This time we look at the two step walk from \(r\)-rank matrix to \(r\)-rank matrix. Let \((N_0,N_2)\) be a an edge in this two step walk and let \(N_1\) be the middle matrix that has rank \(i\). We can sample \((N_0,N_1,N_2)\) by sampling \(N_1' \leq N_1\) of rank \(\frac{r}{3}\). The link graph is (isomorphic to) the two step walk of the graph \(L_{N_1'} = \sett{A \leq M-N_1'}{rank(A)=\frac{2}{3}r}\), \(R_{N_1'}=\sett{B \leq M-N_1'}{rank(B)=i-\frac{r}{3}}\). \Ynote{<<<cite claim later}In the single step version of this walk, we connect \(A\) to \(B\) if \(B \leq A\). Observe that \(i-\frac{r}{3} \leq \frac{1}{3}\cdot \frac{2}{3}r = \frac{2r}{9}\) by assumption that \(i \leq \frac{r}{2}\). By the for every \(N_1'\) the walk \((L_{N_1},R_{N_1})\) is a \(\frac{\sqrt{r}}{\sqrt{3}}2^{\frac{-r}{6}+1.5}\). By \pref{lem:local-to-global} the two step walk is a \(2\frac{\sqrt{r}}{\sqrt{3}}2^{\frac{-r}{6}+1.5} \leq 100r2^{-r/3}\). The claim follows.
\end{proof}

\begin{claim} \label{claim:subposet-link-expansion-full}
    Let \(M\) be a rank \(m\) matrix. Let \(i \leq r\leq m\) such that \(i \leq \frac{r}{2}\) and \(m\geq 2r\). Then \(\lambda(G_{M,r,i}) \leq 10r(2^{-r/6} + 2^{-i})\).
\end{claim}
We note that for every \(\varepsilon > 0\), if \(r \leq (1-\varepsilon) m, i \leq (1-\varepsilon)r\), one should still be able to prof an exponentially decaying bound on the second eigenvalue, but we omit this since it is not important for our work.

\begin{proof}[Proof of \pref{claim:subposet-link-expansion-full}]
    We intend to use \pref{lem:local-to-global} yet again. We analyze the two step walk between \(r\)-rank matrices. for every middle step \(B\), the walk conditioned on \(B\) is isomorphic to \(G_{M,r,i,B} \cong G_{M-B,r-i,0}\). \Ynote{cite claim.}
    By \pref{claim:subposet-graph-no-intersection} this graph is a \(r2^{2(r-i)-(m-i)+2} = r2^{2r-m-i+2} \leq r2^{2-i}\). By \pref{claim:containment-graph-expansion} the walk between \(r\)-rank matrices and \(i\)-rank matrices is a \(10\sqrt{r}2^{-r/6}\) walk. By \pref{lem:local-to-global} this walk has second eigenvalue of \(10r(2^{-r/6} + 2^{-i})\).
\end{proof}

==> Yotam_s_drafts/old/cosystolic_expansion_of_Grassmann.tex <==
\subsection[Local coboundary expansion of the complexes in Golowich 2023]{Local coboundary expansion of the complexes in \cite{Golowich2023}}
In this section we prove that the link of every vertex in the complexes of Golowich \cite{Golowich2023} are coboundary expanders.
\begin{lemma} \label{lem:louis-coboundary-expander}
    Let \(Y=\M(\Gras(\F_2^n)^{\leq d})\) for \(n > 2d\)\Ynote{?}. Let \(X\) be the basification of \(Y\). Then \(X\) has a cone with area \(\Omega(1)\) and is therefore a \(\Omega(1)\)-coboundary expander.
\end{lemma}

The proof of this lemma is a more complicated version of the proof of \pref{lem:cone-for-link-X}. 

Before proving the lemma, let us describe the link structure directly:
\[X(0) = \MP(\frac{d}{2}),\]
\[X(1) = \sett{\set{A_1,A_2}}{\exists B \in \MP(\frac{d}{4}) \; B \oplus (A_1-B) \oplus (A_2-B)}.\]
Finally, the triangles are all \(\set{A_1,A_2,A_3}\) such that there exists \(B_1,B_2,\dots,B_7 \in \MP(\frac{d}{8})\) such that \(\bigoplus_{j=1}^7 B_j\) are a direct sum, and
\[A_1 = B_1\oplus B_2 \oplus B_3 \oplus B_4,\]
\[A_1 = B_1\oplus B_2 \oplus B_5 \oplus B_6,\]
\[A_1 = B_1\oplus B_3 \oplus B_5 \oplus B_7.\]

This description is a direct consequence of the definition of admissible functions in \pref{sec:construction-subpoly-HDX}.

Following the footsteps of the proof of \pref{lem:cone-for-link-X}, we begin with the following two claims. The first bounds the diameter of the underlying graph. This was immediate in the Johnson case but needs to be argued here. This claim also contains a statement on the structure of \(2\)-paths between matrices that are a direct sum. We also require this claim in the analysis.
    \begin{claim} \label{claim:louis-link-const-diam}
        \begin{enumerate}
            \item For any two matrices \(A,B \in X(0)\) there is a path of length \(4\) between \(A\) and \(B\).
            \item If \(A \oplus B\) then there is a path \((A,C,B)\). The middle vertex \(C = A_1 \oplus B_1\) where the components of this sum have equal rank and \(A_1 \leq A\) and \(B_1 \leq B\).
        \end{enumerate} 
    \end{claim}
The second claim is a a variant of \pref{claim:contracting-almost-disjoint-4-cycles-link-X}. \pref{claim:contracting-almost-disjoint-4-cycles-link-X} bounds \(4\)-cycles in the Johnson complex provided that two non-neighboring vertices are disjoint. This claim is the equivalent variant for \(X\):
\begin{claim} \label{claim:tiling-louis-special-cycles}
        Let \((Z,C,A,D,Z)\) be a \(4\)-cycle with the following properties.
    \begin{enumerate}
        \item The matrices \(Z \oplus A\) are a direct sum.
        \item We can decompose \(C=C_1 \oplus C_2\) and \(D=D_1 \oplus D_2\) such that \(C_1,D_1 \leq Z\) and \(C_2,D_2 \leq A\). 
    \end{enumerate}
    Then the cycle has a tiling with \(O(1)\)-triangles.
    \end{claim}
Both of these claims are proven after the lemma.

\begin{proof}[Proof of \pref{lem:louis-coboundary-expander}]
    Observe that the complex \(X\) has a transitive action on the triangles, so it suffices to find a cone whose area is \(O(1)\).
    
    Let \(M_0\) be an arbitrary matrix we take as the root of our cone. We also take length \(4\) paths from \(M_0\) to any matrix \(A \in X(0)\). This is possible by \pref{claim:louis-link-const-diam}.

    For every edge \(\set{A,B}\), the cycle induced by this edge and the paths from \(M_0\) to \(A\) and to \(B\) has length \(9\). Therefore it suffices to show that every \(9\) cycle has a tiling with \(O(1)\) triangles. We begin by reducing the problem into tilings of \(5\) cycles instead. Indeed, observe that for every edge \(\set{C,D}\) in the path, \(\dim(\row(C)+\row(D)) = \dim(\col(C)+\col(D)) \leq \frac{3d}{4}\). Therefore there exists some \(Z \in X(0)\) such that \(\row(Z)\) and \(\col(Z)\) are a direct sum with \(\row(C)+\row(D)\) and \(\col(C)+\col(D)\) respectively (In fact, a random matrix \(Z\) will satisfy this with high probability for all edges in the cycle because \(n \geq 2d\)).

    By \pref{claim:louis-link-const-diam} there exists a length two path from \(Z\) to every vertex \(A\) in the cycle, as in \pref{fig:five-cyc-1}. \Ynote{new figure.}Therefore, by drawing these paths we can decompose our cycle into \(9\) cycles of length \(5\) of the form \((Z,C_1,A_1,A_2,C_2,Z)\) such that the row/column spaces of \(Z\) are a direct sum with \(\row(A_1)+\row(A_2)\) and \(\col(A_1)+\col(A_2)\).

    Fix a cycle as above let us denote by \(B\) the matrix such that \(B \oplus (A_1-B) \oplus (A_2-B)\). Let \(Z_1,Z_2\) be of equal rank such that \(Z = Z_1 \oplus Z_2\). Denote by \(D = Z_1 \oplus B\). We observe that \(\set{Z,D},\set{A_1,D}\) and \(\set{A_2,D}\) are all edges and therefore we can decompose this cycle into a \(3\)-cycle \((D,A_1,A_2,D)\) and two \(4\)-cycles \((Z,C_i,A_i,D,Z)\) (see \Ynote{second new figure}), which we need to tile.

    The tiling of \((D,A_1,A_2,D)\) is simple. We decompose \(Z_1,B,A_1-B\) and \(A_2-B\) into a direct sum of matrices of equal rank \(Z_1=K_1 \oplus K_2, B=L_1\oplus L_2, A_1-B=M_1 \oplus M_2\) and \(A_2-B=N_1 \oplus N_2\). To triangulate we observe that the matrix \(K_1\oplus L_1 \oplus M_1 \oplus N_1\) is connected in a triangle with all three edges.

    As for the cycles \((Z,C_i,A_i,D,Z)\), we tile them with the claim \pref{claim:tiling-louis-special-cycles} and conclude.
\end{proof}

\begin{proof}[Proof of \pref{claim:louis-link-const-diam}]
    First note that the first statement follows from the second, because for any \(A,B\) there exists some \(D \in X(0)\) such that \(A \oplus D\) and \(B \oplus D\) (this is because of the assumption that \(n > 2d\)). Thus we can take a \(2\)-path from \(A\) to \(D\) and then another \(2\)-path from \(D\) to \(B\). 
    
    Let us thus show that assuming that \(A \oplus B\) there is a \(2\)-path from \(A\) to \(B\). Decompose \(A=A_1\oplus A_2\) of equal rank, and similarly for \(B=B_1 \oplus B_2\). Let \(C=A_1\oplus B_1\) and take the path \((A,C,B)\). The claim follows.
\end{proof}

Up until now, this was largely similar to \pref{lem:cone-for-link-X}. Surprisingly, the proof of \pref{claim:tiling-louis-special-cycles} is more complicated then its Johnson analogue \pref{claim:contracting-almost-disjoint-4-cycles-link-X}. This stems from the fact the matrix poset is different from the matrix domination poset, and in particular there isn't a perfect analogue to set intersection in the matrix poset (this is called a meet in poset theory).

\begin{proof}[Proof of \pref{claim:tiling-louis-special-cycles}]
    We will use the middle path pattern \pref{claim:middle-path}. We observe that \(C_1,D_1 \leq Z\) and \(D_2,D_2 \leq A\), and we can view them as vertices in \(\under^{Z}\) and \(\under^{A}\) respectively. We will use a similar strategy as in \pref{claim:contracting-almost-disjoint-4-cycles-link-X}, and use the fact that the graph \(\under^{Z}\) has short paths between every two matrices. That is,
    \begin{claim}\label{claim:short-paths-in-under-graph}
        For every two matrices \(C,D \in \under^m\) there is a path of length \(12\) between \(C\) and \(D\).
    \end{claim}
    This claim is proven in \Ynote{?}. 
    
    Using this claim, we find a pair of \(12\)-paths from \(C_i\) to \(D_i\) in \(\under^{Z}\) and \(\under^{A}\) respectively: \((C_1,M^1,M^2,\dots,M^{11},D_1)\) and \((C_2,N^1,N^2,\dots,N^{11},D_2)\). Then we observe that the matrices \(K^i=M^i \oplus N^i\) form a path \((C,K^1,K^2,\dots,K^{11},D)\) from \(C\) to \(D\) in \(X\). Moreover, every edge in this path is in a triangle with \(A\) and with \(Z\). The claim is proven.
\end{proof}


\begin{proof}[Proof of \pref{claim:tiling-louis-special-cycles}]
    We will use the middle path pattern \pref{claim:middle-path}. We observe that \(C_1,D_1 \leq Z\) and \(D_2,D_2 \leq A\), and we can view them as vertices in \(\under^{Z}\) and \(\under^{A}\) respectively. In particular, we will find a pair of \(12\)-paths from \(C_i\) to \(D_i\) in \(\under^{Z},\under^{A}\) respectively, \((C_1,M^1,M^2,\dots,M^{11},D_1)\) and \((C_2,N^1,N^2,\dots,N^{11},D_2)\). Then we observe that the matrices \(K^i=M^i \oplus N^i\) \((C,K^1,K^2,\dots,K^{11},D)\) is a path from \(C\) to \(D\) in \(X\). Moreover, every edge in this path is in a triangle with \(A\) and with \(Z\).

    Thus, we need to prove that for every two matrices \(C_1,D_1 \in \under^{Z}\) there is a path of length \(6\) from \(C_1\) to \(D_1\) (and similarly for \(\under^{A}\)). We note that \(\under^Z\) and \(\under^A\) are isomorphic so it suffices to do so for one. Let us rename these matrices \(C,D\).

    To do so, we use the following auxiliary claim
    \begin{claim} \label{claim:connecting-disjoint-matrices-in-under-graph}
    \begin{enumerate}
        \item Let \(A,B \in \under^{Z}\) be such that \(\rank(A)=\rank(B) \leq \frac{1}{4}\rank(Z)\). Then for every integer \(r \leq \frac{1}{4}\rank(Z)\) there is a matrix \(T\) with \(\rank(T)=r\) such that \(A \oplus T, T \oplus B \leq Z\).
        \item If \(\rank(A)=\rank(B) \leq \frac{1}{3}\rank(Z)\) then there exists \(M_1,M_2,M_3\) such that
        \[A \oplus M_1, M_1 \oplus M_2, M_2 \oplus M_3, M_3 \oplus B \leq Z.\]
    \end{enumerate}
        
    \end{claim}

    We proceed as follows. We first decompose \(C,D \in \under^Z\) into equal ranked parts \(C=C^1 \oplus C^2\) and \(D=D^1 \oplus D^2\). Then we find some \(T\) of rank \(\frac{d}{8}\) such that \(T \oplus C^1, T \oplus D^1 \leq Z\). This is possible due to the first item in \pref{claim:connecting-disjoint-matrices-in-under-graph}.

    Then we will prove that there exists a \(12\)-path composed of three paths of length \(4\): one from \(C^1\oplus C^2\) to \(C^1 \oplus T\), one from \(C^1 \oplus T\) to \(D^1 \oplus T\) and one from \(D^1 \oplus T\) to \(D^1 \oplus D^2\).

    Let us show how to construct the first path, the other two are constructed similarly. Note that \(C^1 \leq C^1 \oplus C^2, C^1 \oplus T\) and that they are both \(\leq Z\). Thus if we find \(M^1,M^2,M^3 \leq Z-C^1\) such that
    \[C^2 \oplus M^1, M^1 \oplus M_^2, M^2 \oplus M^3, M^3 \oplus T \leq Z - C^1,\]
    Then by \pref{prop:iso-of-posets}, adding \(C^1\) to all three \(M^1,M^2,M^3\) will give us the desired path in \(\under^Z\):
    \[(C^1\oplus C^2,C^1\oplus M^1, C^1\oplus M^2, C^1\oplus M^3, C^1\oplus T).\]
    But observe that existence of such matrices \(M^1,M^2,M^3\) is promised by \pref{claim:connecting-disjoint-matrices-in-under-graph} so we can conclude.
\end{proof}

\begin{proof}[Proof of \pref{claim:connecting-disjoint-matrices-in-under-graph}]
    \Ynote{If this ends up not being part of the appendix we should make this a claim:}Without loss of generality let us assume that \(Z = I\) the identity matrix of rank \(\rank(Z) = \ell\). Recall that in \pref{claim:base-case} we saw the observation of \cite{Golowich2023} that \(A \leq I\) if and only if \(A = \sum_{i=1}^{\ell''} e_i \otimes f_i\) for some \(\ell'' \leq \ell\) and \(\set{e_i}_{i=1}^{\ell''},\set{f_i}_{i=1}^{\ell''}\) such that
    \[\iprod{e_i,f_j} = \begin{cases}
        1 & i=j \\
        0 & i \ne j
    \end{cases}.\]

    Let us begin with the first item. Given \(A,B\) of rank \(\leq \frac{1}{4}\ell\) we need to find some \(T\) of tank \(\leq \frac{1}{4}\ell\) such that \(A \oplus T, B \oplus T \leq Z\). Without loss of generality, we assume that \(\rank(A)=\rank(B)=\frac{1}{4}\ell\) and find \(T\) of rank \(\frac{1}{4}\ell\) with the desired property. 
    Let us write \(A = \sum_{j=1}^{\ell/4} e_j(A) \otimes f_j(A), B=\sum_{j=1}^{\ell/4}e_j(A) \otimes f_j(A)\). We begin by finding independent \(e_1(T),e_2(T),\dots,e_{\ell/2}(T) \in \F_2^\ell\) such that \(\iprod{e_i(T),f_j(A)}=\iprod{e_i(T),f_j(B)} = 0\) for every \(i,j\). We can do so since \(\iprod{x,f_j(A)}=0, \iprod{x,f_j(B)}=0\) are \(\leq \frac{2}{3}\ell\) equations.

    Now let \(W = \sp(e_1(T),e_2(T),\dots,e_{\ell/2}(T))\). We note that \(W \cap \row(A)=W \cap \row(B) = \set{0}\). Let us show this for \(\row(A)\): for any non-zero vector from \(x\in \row(A)\) is a sum of \(\sum_{j=1}^{\ell/3} b_j e_j(A)\) where at least on of the \(b_j\)'s are not zero. On the other hand, \(\iprod{x,f_j(A)} = b_j\), so there is at least one \(\iprod{x,f_j(A)} \ne 0\), implying that \(x \notin W\). Thus we conclude that \(\dim(W \cap (\row(A) + \row(B))) \leq \frac{\ell}{4}\). Without loss of generality, let \(E = \set{e_1(T),\dots,e_{\ell/4}(T)}\) be such that \(\sp(E)\) intersects trivially with \(\row(A) + \row(B)\).

    In particular, this implies that for every \(i=1,2,\dots,\frac{\ell}{4}\), there exists some \(f_i(T)\) such that \(\iprod{e_j(A),f_i(T)} = \iprod{e_j(B),f_i(T)} = 0\) for all \(j=1,2,\dots,\frac{\ell}{4}\) and in addition
    \[\iprod{e_j(T),f_i(T)} = \begin{cases}
        1 & i=j \\ 0 & i \ne j
    \end{cases}.\]
    By taking \(T = \sum_{j=1}^{\ell/4} e_j(T) \otimes f_j(T)\) we can conclude.
    
    Let us turn to the second item. The strategy here will be similar. We begin by finding \(e_1(M^{1}),e_2(M^{1}),\dots,e_{\ell/3}(M^{1})\) that are independent and perpendicular to all \(f_j(A),f_j(B)\) as before, and also set \(e_j(M^3)=e_j(M^1)\) (we can find such vectors just by the fact that the number of linear constraints is \(\leq \frac{2}{3}\ell\)). Then we find the \(f_j(M^1)\) and \(f_j(M^3)\) where \(f_j(M^1)\) are perpendicular to \(e_j(A)\), \(f_j(M^3)\) are perpendicular to \(e_j(B)\) and
     \[\iprod{e_j(M^1),f_j(M^1)} = \iprod{e_j(M^3),f_j(M^3)} = \begin{cases}
        1 & i=j \\ 0 & i \ne j
    \end{cases}.\]
    Again existence of such vectors is by solving two sets of linear equations with \(\leq \frac{2}{3}\ell\) equations each. Here we also use the fact that the span of the \(e_j(M^1)\)'s is independent from the spans of \(e_j(A)\) (and \(e_j(B)\)) to make sure that there indeed exists a solution.
    
    Then we set \(M^1 = \sum_{j=1}^{\ell/3} e_j(M^1) \otimes f_j(M^1)\) and \(M^1 = \sum_{j=1}^{\ell/3} e_j(M^3) \otimes f_j(M^3)\). It is easy to verify that as before \(A \oplus M^1, B \oplus M^3 \leq Z\).

    Now we find \(M^2\) such that \(M^1 \oplus M^2, M^2 \oplus M^3 \leq Z\). The upshot of the previous step is that now \(M^1\) and \(M^3\) have the same row space \(\sp(\set{e_1(M^1),e_2(M^1),\dots,e_{\ell/3}(M^1)})\). Thus we find \(M^2\) as follows. We start by finding \(e_1(M^2),e_2(M^2),\dots,e_{\ell/3}(M^2)\) by requiring they be independent and such that they are all perpendicular to the \(f_j(M^1)\) and the \(f_j(M^3)\)'s. Then we observe that because they intersect trivially with the row spaces of \(M^1\) and \(M^3\) (as before), we can find \(f_j(M^2)\) such that \(f_j(M^2)\) are perpendicular to the row spaces of \(M^1\) (and \(M^3\)), and such that 
     \[\iprod{e_j(M^2),f_j(M^2)} = \begin{cases}
        1 & i=j \\ 0 & i \ne j
    \end{cases}.\]
    Setting \(M^2 = \sum_{j=1}^{\ell/3} e_j(M^2) \otimes e_j(M^3)\) completes the proof.
\end{proof}

\subsection{Coboundary expansion in the links and cosystolic expansion}
    In \cite{Golowich2023} it is proven that the Cayley complex whose link is \(X\) is not a coboundary expander for any constant \(\beta > 0\). It is done by proving that \(Z^1(X,\Gamma) \ne B^1(X,\Gamma)\).
    
    However, we can still prove that these complexes are \emph{cosystolic expanders}. This notion is a weakening of coboundary expansion that allows the existence of cohomology, i.e.\ for \(Z^1(X,\Gamma) \ne B^1(X,\Gamma)\):
    \begin{definition}[$1$-dimensional cosystolic expander] \label{def:def-of-cosystolic-exp}
        Let \(X\) be a \(d\)-dimensional simplicial complex for \(d \geq 2\). Let \(\beta >0\). We say that \(X\) is a $1$-dimensional \emph{\(\beta\)-cosystolic expander} if for every group \(\Gamma\), and every \(f \in C^1(X,\Gamma)\) there exists some \(h \in Z^1(X,\Gamma)\) such that
    \begin{equation} \label{eq:def-of-cosyst-exp}
        \beta \dist(f,h) \leq \wt(\coboundary f).
    \end{equation}
    \end{definition}
    The difference between this definition and the definition of coboundary expansion, is that in the definition of coboundary expansion we require \(h=\coboundary g\), or equivalently \(h \in B^1(X,\Gamma)\) whereas here we only require \(h \in Z^1(X,\Gamma)\) which is less restrictive.

    We note that cosystolic expansion is still an important property and can sometimes be used in applications such as topological overlap property \cite{DotterrerKW2018} or to get some form agreement testing guarantee \cite{DiksteinD2023agr}.

Kaufman, Kazhdan and Lubotzky were the first to prove that observed that in local spectral expanders, cosystolic expansion follows from coboundary expansion of the links \cite{KaufmanKL2016} (together with local spectral expansion). Later on their seminal result was extended to all groups and higher dimensions \cite{EvraK2016,KaufmanM2018,KaufmanM2021,KaufmanM2022,DiksteinD2023cbdry}. In particular, we can use the quantitatively strong theorem in \cite[Theorem 1.2]{DiksteinD2023cbdry}, to get cosystolic expansion from \pref{lem:louis-coboundary-expander} and the local spectral expansion.
\begin{corollary}
    Let \(X\) be the complex obtained by \Ynote{complete}. Assume that \(n\) is sufficiently large such that \(X\) is a \(10^{-3}\)-local spectral expander. Then \(X\) is also an \(10^{-3}\)-cosystolic expander.
\end{corollary}
We omit the details.

==> Yotam_s_drafts/old/draft1.1.1.tex <==
The first construction we present is a family of Cayley local spectral expanders \snote{Cayley HDXs vs Cayley local spectral expanders?} with subpolynomial degree \(2^{n^\varepsilon}\) where \(N = 2^n\) is the number of vertices. Namely,
\begin{theorem} \torestate{\label{thm:main-recursive-hdx-intro}
    For every \(\lambda, \varepsilon > 0\) and integer \(\diml \geq 2\) there exists an infinite family of \(\diml\)-dimensional Cayley \(\lambda\)-local spectral expanders \(\S\) over $\F_2^n$ with degree at most \(2^{n^{\varepsilon}}\).}
\end{theorem}
This construction builds on an ingenious construction by Golowich \cite{Golowich2023}, which proved this theorem for \(\varepsilon = \frac{1}{2}\). The construction in \cite{Golowich2023} is based on sparsifying the well studied Grassmann poset, the partial ordered of subspaces of \(\F_2^n\), ordered by containment. This object is the vector space equivalent of high dimensional expanders, and was previously studied in \cite{DiksteinDFH2018,kaufmanT2021garland,GaitondeHKLZ2022,Golowich2023}.

One can view the \cite{Golowich2023} construction as a family of complexes arising naturally from a \emph{sparsification} of the Grassmann. The key idea in \cite{Golowich2023} is to sparsify the Grassmann poset to obtain a sub-poset, and afterwards construct the sparse simplicial complex using said sparse sub-poset. Our construction takes a modular approach to this idea. We modify the poset sparsification in \cite{Golowich2023} so that instead of the Grassmann poset, we can plug in \emph{any} subposet \(\Y\) of the Grassmann, and a obtain a sparsification \(\Y'\) whose size depends on \(\Y\) (not the complete Grassmann).

Having this flexible sparsification step, we \emph{iterate}. We start with \(Y_0\), the complete Grassmann poset, we obtain a sequence \(\Y_1,\Y_2,\dots,\Y_m\) of sparser and sparser subposets. Actually, \(\abs{\Y_i} = \abs{Y_0}^{C}\) for some constant \(C > 1\). Similar to \cite{Golowich2023}, we are able to call this `a sparsification' because \(\Y_0\) is the complete Grassmann of subspaces of \(\F_2^n\), but \(\Y_i\) is a subposet of the Grassmann of subspaces of \(\F_2^{n^{2^i}}\). Changing variables to \(n' = k^{2^i}\), we can view \(Y_i\) as a sparsification with \(2^{O(n'^{2^{-i}})}\) subspaces! % Miri Regev: applause.

We comment that while this is a powerful paradigm, it does have a drawback. The dimension of \(\Y_{i}\) is is log the dimension of \(\Y_{i-1}\) (the dimension of \(Y\) is the maximal dimension of a space inside \(\Y\)). Thus we can only continue this sparsification \(O(\log^* k)\)-steps, keeping \(\varepsilon\) essentially constant.

We will now give a high level description of the reduction step. Golowich constructs a sparse Grassmann sub-poset of the Grassmann over \(\F_2^{n}\), by identifying \(\F_2^n = \F_2^{k \otimes k}\) to be \(k \times k\) matrices for \(k=\sqrt{n}\). The one dimensional subspaces are (spans of) the \(2r\)-rank matrices, where \(r\) is some fixed constant. Our change is simple. Given a subposet \(\Y\) of the Grassmann over \(\F_2^{k}\), we produce a subposet \(\Y'\) of the Grassmann over \(\f_2^{k \times k}\), where the \(1\)-dimensional subspaces correspond to matrices of rank \(2r\) \emph{whose row and column spaces belong to \(\Y\)}.

This construction produces local spectral expanders of any constant dimension. The higher dimensional subspaces of \(\Y'\), that correspond to the higher dimensional faces in the resulting simplicial complex, are the correct analogue of \cite{Golowich2023}, and we refer the reader to \pref{sec:construction-subpoly-HDX} for more details. The analysis of the local spectral expansion is delicate, so we will not describe it here. It builds upon the machinery of \cite{Golowich2023}, in addition to a local-to-global component we wish to highlight. This component is a local to global decomposition given in \cite{Madras2002}, that is in the spirit of Garland's method \cite{Garland1973}.

Given a graph \(G = (V,E)\) that we wish to analyze, we find a set of expanding subgraphs \( \set{H_1, H_2, \dots H_m}\) of \(G\) (that are allowed to overlap). We show that if every \(H_i\) is an expander and the walk that goes from vertex to vertex if they share a subgraph is also an expander, then \(G\) is an expander. We call this the `local-to-global' graph.

This local-to-global decomposition is particularly useful in our setup. The graphs we need to analyze in order to prove the expansion of our complexes, can be decomposed into smaller subgraphs \(H_i\) that are isomorphic to graphs coming from the original construction of \cite{Golowich2023}. Using this decomposition we are able to relate the `local-to-global' graph to containment graphs in \(\Y\), which are known to be excellent expanders.

==> Yotam_s_drafts/old/intro_me.tex <==


The first definition of high dimensional expansion is a local one. A simplicial complex \(X\) is a \(\lambda\)-\emph{local spectral expander} if it is connected (as a graph \((X(0),X(1))\)) and for every \(v \in X(0)\), \(X_v\) is a \(\lambda\)-two-sided spectral expander.\footnote{That is, the second largest eigenvalue of the random walk operator of \(X_v\) is \(\leq \lambda\) in absolute value.} This seemingly naive definition is quite strong: for example it strong enough local spectral expansion implies expansion of the underlying graph of \(X\). In higher dimensions it implies non-trivial structure such as hypercontractivity, a Fourier decomposition, and concentration of measure \Ynote{cite}. Spectral expansion has found many uses in theoretical computer science and geometry, such as \Ynote{complete}.

\Ynote{need to complete definition.}
The second important definition is somewhat more mysterious. The simplest way to define it is through property testing of partitions. 

Even though this definition is less clear, it implies robust topological properties of the complex. These include cover testability, topological overlap properties (a strong non-embedability of the complex in \(\R^2\)). It is connected to low-rank matrix testing, quantum codes, and with the recent results of agreement testing.

Constructing bounded degree complexes satisfying both definitions is an important goal in the high dimensional expander community. Local spectral expanders were first constructed in a series of works on quotients of Bruhat-Tits buildings \Ynote{all the citations}. Other bounded degree constructions also use non-trivial group theory \Ynote{cite}. Constructions that do not use number theory include \Ynote{complete}. The state of the art, is an elegant construction by Golowich giving a family of \(\lambda\)-local spectral expanders whose degree is \(2^{O_\lambda(\sqrt{\log |X(0)|})}\) (subpolynomial, but far from constant or even \(\polylog\)) \cite{Golowich2023}\footnote{To be clear, the degree of a vertex is the number of edges adjacent to it.}. We will elaborate on this construction later in the introduction. This raises natural questions: how complex are families of bounded degree high dimensional expanders? Is there a random distribution for bounded degree high dimensional expanders?

If we require both coboundary expansion and spectral expansion, the situation is even worse. There are no known coboundary expanders of bounded degree. As far as we know, the state of the art is random complexes which have an average degree of \(|X(0)|^{2/3}\) \Ynote{cite kahle}. All previous constructions are known to \emph{not} have coboundary expansion. Although there are more relaxed definitions that allow for some of the applications, the question remains whether there exists a family of bounded degree spectral and coboundary expanders.

\subsection{Our results}
In this work we present two constructions of high dimensional expanders whose underlying graph is a Cayley graphs of \(\F_2^n\). The first construction, is an improvement of the construction by \cite{Golowich2023}. For every \(\varepsilon, \lambda > 0\) and dimension \(d\), we construct a family of \(d\)-dimensional \(\lambda\)-local spectral expanders. The vertex degree in this construction is  \(2^{O_{d,\lambda}(\log |X(0)|)^{\varepsilon}}\). Although still much larger than \(\polylog\)-degree.
\Ynote{maybe write down the theorem here.}

Our second construction is a higher degree local spectral expander that is also a coboundary expander. While we do not control the degree as in the first construction, we can still expansion below the ``trickle down barrier'' for any polynomial degree \(|X(0)|^\varepsilon\). Let us explain this sentence. The trickle-down theorem mentioned above states that a \(\lambda\)-high dimensional expander has a \(\frac{\lambda}{1-\lambda}\)-expanding underlying graph \Ynote{cite oppenheim} (building upon the Garland method \Ynote{cite Garland}). This is meaningful for \(\lambda < \frac{1}{2}\). As noticed in \Ynote{cite Chapman and Golowich}, this theorem is also a barrier, and constructing local spectral expanders with \(\lambda < \frac{1}{2}\) is a significantly more challenging task. The known combinatorial constructions all achieve \(\lambda = \frac{1}{2}\) but not lower \Ynote{cite}.

Known constructions beating the barrier are the bounded degree construction mentioned above, Golowiches construction and Random geometric graphs. All but the later are known \emph{not} to be coboundary expanders for \emph{any} constant above \(0\); the coboundary expansion of the random geometric graphs is not known.

We prove the following theorem.
\Ynote{Theorem about Johnson.}
This matches the degree of \Ynote{RGG}, and is simple enough to analyze the coboundary expansion.

This paper will focus on highly symmetric graphs and complexes arising from groups. We call \(X\) a Cayley complex if its skeleton \(G\) is a Cayley graph \(G=Cay(H;S)\), with vertices labeled by the elements of some finite group \(H\), and its edges describe multiplication by a \emph{generator} from some symmetric \footnote{If \(s\in S\) also \(s^{-1} \in S\), so the resulting graph is undirected.} set \(S \subseteq H\) of generators (in this case the degree \(D=|S|\)). Note that a Cayley graph is vertex transitive (by the natural action of \(H\) on itself), and so in particular all links are isomorphic. In this work, we will mainly study expansion properties of Cayley graphs on the group \(H=\F_2^n\).



Of central importance is the degree \(D\) of the graph \(G\) (for simplicity we would also assume that \(G\) is regular, namely that every vertex has exactly \(D\) neighbors, and also that every edge is on the same number of triangles). The sparsity of \(X\) depends on the relation of the degree \(D\) and the size $N=|V|$. While most existing applications focus on the case where \(D\) is an absolute constant, independent of \(N\), in some situations this is impossible to achieve (e.g. where we must have \(D > \log N\))\Ynote{sentence not clear without more context}. Thus, some works we follow have studied regimes where \(D\) is polynomial in \(N\) (e.g. \(D=N^\varepsilon\)) or subpolynomial in \(N\) (e.g. \(D=N^{o(1)}\)).



There are two main notions of expansion of such a complex, spectral and (the more combinatorial/geometric) coboundary expansion, and we will separate the discussion of each.

\subsection{Spectral expansion}
%
The spectral expansion of a a graph \(G\) is measured by the \(2\)-nd largest eigenvalue of its random walk matrix, denoted \(\lambda(G)\), which is bounded away from \(1\) independently of the graph size \(N\).\Ynote{make more formal} One can (and does) consider the expansion of a complex \(X\) via its underlying 1-skeleton \(G_X\), and denote \(\lambda(X)=\lambda(G_X)\). In fact, a variety of notions of spectral expansion of higher dimensional complexes was developed since the original Ramanujan complexes of [LSV], but the field has converged on one which seems the most useful in applications, namely the \(2\)-nd eigenvalue of its links. For a complex \(X\) we let \(\lambda_L(X)\) denote the largest \(2\)-nd eigenvalue of all possible links \(L(v)\) with \(v\in V\) (note that for Cayley complexes all these values are equal). 

A central feature of high-dimensional expanders is their \emph{local-to-global} property: if all links are \emph{very} good expanders, then the whole complex is expanding. More precisely, for 2-dimensional complexes, if \(\lambda_L(X) = \alpha\), then \(\lambda(X) \leq \alpha / (1-\alpha )\). More precisely, if we have a constant gap \(1/2 - \alpha >0\), a local property of the links, we immediately get that globally the whole complex $X$ is an expander!\Ynote{cite oppenheim}\footnote{For higher, \(k\)-dimensional complexes we have a similar property, which we formally state in the technical part. Essentially, a bound of \(< 1/k\) on the eigenvalue of \(1\)-dimensional links of \(k-2\)-dimensional faces implies global expansion at all levels of \(X\).}\footnote{To see that the bound 1/2 is best possible consider the Cayley graph \(Cay(H,S)\) with \(H=\F_2^n\) and \(S\) is all \(n\)-vectors of Hamming weight 2. Note that every link is isomorphic to the line graph of the complete graph \(K_n\), whose 2nd eigenvalue is \(1/2-1/n\).}  This understanding originates from the work of Garland [G] on buildings, continues with Zuk's [Zuk] work on infinite expanding random groups, and elucidated clearly and in general for finite complexes by Oppenheim [Opp] \Ynote{I think we should be more generous toward Oppenheim}. This ``trickle-down" property was responsible to the new breakthroughs in the analysis if Markov chains (starting from [LSTV]), and is the primary method by which spectral expansion of complexes is proved. For this reason, we will not survey below many constructions (eg [Conlon],[Linial-..]) of complexes, interesting for other reasons,  in which \(\lambda_L(X) \geq 1/2\). 

This condition of making all links excellent expanders is what explains some of the magic of HDX as well as the difficulty of finding them, probabilistically or deterministically. After all, expansion of a graph entails local sparsity, whereas expansion of links entails local density. For example, a random sparse graph will have \emph{no} edges at all in any link, but will still be an excellent global expander almost surely. If we insist on bounded degree \(D\) local density seems especially demanding. Indeed, there are only a handful of essentially different constructions [CSZ03, Li04, LSV05a, LSV05b, KKL14, KO18, OP22] (refs from Siqi's geometric exp paper). All of these constructions are algebraic, obtained as Cayley graphs of quotients of certain infinite groups of special structure. No combinatorial construction of this type was found despite nontrivial effort.

Even allowing \(D\) to grow with \(N\) leaves this problem quite difficult until the graph is quite dense. It is easy to see that when \(D  = \Omega (N^{1/2}\log N)\), a random graph of average degree \(D\) will have excellent link expansion almost surely. The reason is that the birthday paradox happens, and the links will be themselves random graphs with logarithmic degree. Indeed, this works also for Cayley graphs! Take \(Cay(H;S)\) with any group \(H\) of size \(N\) and \(D\) (as above) subset \(S\) at random, and the links will be highly expanding. This is essentially the argument of [Zuk] in his random construction of infinite random (hyperbolic) groups with property (T)\footnote{The infinite analog of expansion.}, and the analysis of this statement is almost as simple as for general graphs. 

But what about smaller densities? Obtaining elementary explicit constructions of density below \(D = o(N^{1/2})\), or natural probability distributions on graphs with such densities with expanding links has been out of reach until two breakthroughs in the past couple of years ago. In both, beautiful new ideas and analytic tools were introduced to the HDX field, that have surely enriched it. We now exposit both in turn, as well as our improvements on each.  

\subsubsection{Explicit construction of subpolynomial density}

Only a few months ago\Ynote{more than a year ago?}, Golowich [Gol23] put forward an ingenious construction of HDX (of any constant dimension!)\footnote{Though we will describe here only the 2-dimensional one.}  of size \(N\) with very subpolynomial degree \(D= \exp(\log N)^{1/2}\). There are several ways of looking at this construction which are detailed in this paper, which are important to certain structural applications, and we choose the simplest one to describe. This construction is actually a Cayley complex, of the Abelian group \(\F_2^n\). It is obtained as a \emph{sparsification} (or \emph{derandomization}) of the trivial, \emph{complete} graph on this group, in which all pairs of elements are connected (needless to say, this is the best possible HDX, as all links are complete graphs as well). The key is taking a somewhat strange-looking view of this object.

Assume \(n=k^2\), and identify \(\F_2^n\) with \(\F_2^{k \times k}\), the space of \(k\times k\) matrices over \(\F_2\). Golowich sparsifies this complete graph by restricting the generating set from all matrices, to the set \(S\) of matrices of some \emph{constant} rank \(2r\). Note that the number of such matrices is only \(D= \exp(O(k))\), while the graph has size \(N = \exp(2^{k^2})\), satisfying the required sparsity. The analysis is subtle, and we cannot do it justice in this introduction, but we want to highlight two key ideas which are essential for us as well. The first idea has to do with richness of representations of matrices. Note that there are many ways in which any rank-\(2r\) matrix \(A\) can be written as the sum of two rank-\(r\) matrices, say \(M_1\) and \(M_2\), and many ways to pick another rank-\(r\) matrix \(M_3\) so that the sum \(M_2+M_3=B\) has rank \(2r\), and so \(C=A+B\) is a neighbor of \(A\) in the link.  Moreover, each rank-\(2r\) matrix, say \(A\), has many representations \(A=ST\) with \(S\) being \(k \times 2r\) and \(T\) being \(2r \times k\), coming from (coordinated) choices of bases for row and column \emph{subspaces}, and so the choice of partition \(A=M_1+M_2\) is far richer than simply partitioning a set of size \(2r\) to two sets of size \(r\). The second idea is to use another type of complex. If simplicial complexes ``live" in the poset if \emph{subsets} of a set, \emph{Grassmann} complexes ``live" in the poset of \emph{subspaces} of a vector space.  Grassman complexes were studied, and for example it is known that they possess a similar ``trickle-down" local-to-global property as simplicial complexes [Tali-??]. The richness of representation and properties of Grassmann complexes\footnote{Observe another subtlety - here we really have a product of two Grassman complexes, one for the rows and one for the columns.}   allow Golowich to prove that this ``derandomization" of the complete graph works, and hence that  this radical sparsification of edges essentially maintains the expansion of the original complete complex with small, quantifiable loss.  

We develop Golowich's ideas further and show that similar techniques can actually be used to derandomize not only the compete complex. Indeed, we prove that they a large family of sufficiently expanding simplicial complexes\footnote{Of high enough constant dimension!} which is similarly based on Grassman complexes. And moreover, a particular member of this family is Golowich' complex above. This allows us to iterate his construction, repeatedly sparsifying the generating sets to obtain expanding Cayley complexes over \(\F_2^n\) with degree \(D=\exp(\log N)^\epsilon\) for any \(\epsilon\).

\begin{theorem}
    Fix any \(\epsilon, \alpha >0\), and dimension \(d\). For every \(n\) we explicitly construct a subsets \(S_n\) of size \(D_n = \exp(n^\epsilon)\) such that the Cayley graphs \(Cay(\F_2^n, S_n)\) is a dimension \(d\) and link expansion at most \(\alpha\). \Ynote{not sure what this comment means:[We can of course get much smaller e-values]}.
\end{theorem}

==> Yotam_s_drafts/old/lower_bound_Cayley_complexes.tex <==
\section{A degree lower bound}
    A classical result in graph theory says that a connected Cayley graph over \(\F_2^n\) has degree at least \(n\). In this section we prove that Cayley HDXs have degree at least \(1.5 n\), based on the code theoretic interpretation of the links given in \cite{Golowich2023}[Lemma 77]. A link in a Cayley complex \(X\) naturally comes with labels on the edges which are induced by the generating set (i.e.\ an edge between \(x+s_1\) and \(x+s_2\) in the link of \(x\) will be \(s_1+s_2\) which by assumption is a generator in the generating set). Note that if \(x+s_1,x+s_2\) is labeled \(s_1+s_2\) then there is a \(3\)-cycle in the link between \(x+s_1,x+s_2\) and \(x+s_1+s_2\) where every edge that corresponds to two generators is labeled by the third generator.

Let \(G=(V,E)\) be a graph with vertex set \(V=\set{v_1,v_2,\dots,v_m}\) and a labeling \(\ell:E \to V\). The graph \(G\) is \emph{nice} if for every \(\set{v_i,v_j}\) that is labeled \(v_k\) there is a three cycle \(v_i,v_j,v_k\) in the graph where \(\set{v_i,v_k}\) is labeled \(v_j\) and \(\set{v_j,v_k}\) is labeled \(v_i\). We would like to understand for which \(n\) does there exist a Cayley complex \(X\) so that a link \(X\) is isomorphic to \(G\). That is, for which \(n\) can we find generators \(s_1,s_2,\dots,s_m \in \F_2^n\) such that the map \(\phi(s_i)=v_i\) is a label graph isomorphism. Observe that for this to hold, whenever there is an edge \(\set{v_i,v_j} \in E\) labeled by \(v_k\), we require  that \(s_i+s_j+s_k = 0\). Thus we can define the matrix \(H_G \in \F_2^{|E| \times |V|}\) to have in every row the indicator vector of \(i,j,k\) for every \(\set{v_i,v_j} \in E\) labeled by \(v_k\). Let us show that this is a sufficient condition.

The following is essentially observed in \cite{Golowich2023}[Lemma 77].
\begin{claim}
    Let \(G\) be a nice graph with \(m\) vertices. Let \(S = \set{s_1,s_2,\dots,s_m} \in \F_2^n\) and let \(M_s\) be the matrix whose rows are the \(s_i\)'s. Then the following is equivalent.
    \begin{enumerate}
        \item The columns of \(M_s\) are in the kernel of \(H_G\).
        \item There exists a Cayley complex \(X\) over \(\F_2^n\) whose link is isomorphic to \(G\) whose underlying graph is \(Cay(\F_2^n,S)\).
    \end{enumerate}
    In particular, if the above occurs and the Cayley complex is connected then 
    \(m \geq n + \rank(H_G)\).
\end{claim}

\begin{proof}
    If the first item occurs, then this means that for every \(\set{v_i,v_j} \in E\) labeled by \(v_k\), \(s_i+s_j+s_k = 0\) and therefore the \(3\)-cycles \((x,x+s_i,x+s_i+s_j=x+s_k,x)\) are in \(Cay(\F_2^n,S)\) so we can take \(\set{x+s_i,x+s_j,x+s_k}\) into our set of triangles. The isomorphism of the link of \(X\) to \(G\) is direct to check.

    On the other hand, from the discussion above, the isomorphism to \(G\) implies that every triangle \(\set{v_i,v_j}\) labeled \(v_k\) implies that \(s_i+s_j+s_k = 0\) hence the columns of the matrix are in \(Ker(H_G)\).

    In particular, this implies that \(\rank(M_s) \leq \dim(Ker(H_G)) = m-\rank(H_G)\). On the other hand, if the complex is connected then \(\rank(M_s) \geq n\). Combining the two we get that the degree, \(m \geq n+\rank(H_G)\).
\end{proof}

\begin{corollary}
    Let \(X\) be a connected Cayley complex with degree \(m\) such that the link of \(X\) contains no isolated vertices. Then \(m \geq 1.5 (n-1) \).
\end{corollary}

\begin{proof}
    The corollary follows from the inequality \(m \geq n+\rank(H_G)\), together with the observation that \(\rank(H_G) \geq \frac{m}{3}\) which we now explain. We can greedily select independent rows from \(H_G\) such that whenever a generator \(s_i\) appears in no equation, we take an equation (or row) where \(s_i\) appears. As every equation covers \(3\) new variables at most, we can find at least \(\frac{m}{3}-1\) such equations. Thus,
    \(m \geq n+\frac{m}{3}-1\) and the bound follows.
\end{proof}


==> Yotam_s_drafts/old/old_roadmap.tex <==
\subsection{A Proof Roadmap for the Recursion Theorem - \pref{thm:one-step-of-recursion}} \label{sec:proof-roadmap}
The rest of this section is devoted to proving \pref{thm:one-step-of-recursion}, and mainly to bounding the expansion of \(\Y'\). 

We fix the parameters \(\lambdao\) and \(\dimlout\). Without loss of generality we take \(\dimlout\) to be large enough so that \(\dimlin = 2^{2\dimlout}\). This requires that \(\dimlout \geq \log K + \log \log \frac{1}{\lambdao}\) for the constant \(K > 0\) that we do not calculate explicitly in \pref{thm:one-step-of-recursion}. %This is always possible since we can always take a lower dimensional skeleton of \(\Y'\) instead of \(\Y'\) itself.

Here we also recall the partial order defined in \pref{sec:def-of-domination-relation} on matrices where we write \(A \leq M\) for two matrices \(A,M \in \F_2^{n \times n}\) if \(\rank(M) = \rank(A) + \rank(M-A)\). %In \pref{app:removing-lower-matrix} we prove some properties we need of this partial order, required later.

\medskip

Fix \(\Y\), \(\Y' = \M(\Y)\) and a subspace \(U \in \Y'(\dimm)\) (where \(\dimm \leq \dimlout\)). The main effort in will be to prove that the link \(\Y'_U\) is sufficiently expanding.

\paragraph{Step \(I\)}We will show that a link of a subspace \(U \in \Y'(\dimm)\) decomposes to a tensor product of simpler components. For this it will be more convenient to consider the \emph{augmented link graph}.

\begin{lemma}\label{lem:grassmannian-link-decomposition}~
  \(\Y'_U \cong \underbrace{(G_\dimm \otimes G_\dimm \otimes \dots \otimes G_\dimm)}_{2^\dimm -1 \text{ times}} \otimes \SL(\Y,U)\).
\end{lemma}
which we now define. For the rest of this section let \(m = \frac{\dimlin}{2^{\dimm+2}}\).
\begin{definition}[Subposet Graph] \label{def:subposet-graph}
    Let \(M\) be a rank \(4m\) matrix. The graph \(G_\dimm(M)\) has vertex set
    \[V = \sett{A \leq M}{\rank(A) = 2m}.\]
    We connect \(A_1\) and \(A_2\) if there is a decomposition \(M = B_1 \oplus B_2 \oplus B_3 \oplus B_4 \) such that every \(B_i\) has rank \(m\), \(A_1 = B_1 \oplus B_2\) and \(A_2 = B_2 \oplus B_3\).
\end{definition}
The graphs \(G_\dimm(M), G_\dimm(M')\) are isomorphic for every two \(M,M'\) of rank \(m\), hence we denote them \(G_\dimm\) when we don't care about \(M\). %We observe that the graph \(\mathcal{S}^M(\frac{m}{2},\frac{m}{2},\frac{m}{4})\) is the double cover of \(G_\ell(M)\), thus by \pref{lem:expansion-of-S-upper-loc}, \(\lambda(G_\ell) \leq 2^{-\alpha m}\)-spectral expander.

The second graph has a similar rule for connecting edges, but a different vertex set.
\begin{definition}[Sparsified link graph] \label{def:sparsified-link-graph}
   Let \(S_U\) be the unique matrix corresponding to \(U\) as in \pref{def:matrix-poset}.% and let \(w_R = \row(S_U)\) and \(w_C=\col(S_U)\).
   The graph \(\SL(\Y,U)\) is the graph with vertex set
    \[ V = \sett{A \in \MP_{\cap S_U}(2m)}{\row(A) \oplus \row(S_U), \; \col(A) \oplus \col(S_U)  \in \Y\left(\dimlin-2m \right)}.\]
    The edges are all \(A_1,A_2\) such that there exists a matrix \(M\) of rank \(4m\) such that \(\row(M) \oplus \row(S_U), \; \col(M) \oplus \col(S_U) \in \Y\), and \(\set{A_1, A_2}\) are an edge in \(G_\dimm (M)\).

Moreover, we also denote \(L(\Y_1,\Y_2,U)\) the same graph as above with the distinction that we require \(\row(A) \oplus \row(S_U) \in \Y_1\) and \(\col(A) \oplus \col(S_U)  \in \Y_2\) (and similarly for the edges).
\end{definition}
We comment that formally, the distribution over edges in the sparsified link graph \(L(\Y,U)\) is the following. %Let \(w_R = \row(S_U)\) and \(w_C = \col(S_U)\):
\begin{enumerate}
    \item Sample \(w_1 \in Y_{\row(S_U)}(\dimlin)\) and \(w_2 \in Y_{\col(S_U)}(\dimlin)\) according to the respective distributions of \(Y_{\row(S_U)}(\dimlin),Y_{\col(S_U)}(\dimlin) \).
    \item Uniformly sample a matrix \(M\) %of rank \(4m\) 
    such that \(\row(S_U) \oplus \row(M) = w_1\) and \(\col(S_U) \oplus \col(M) = w_2\) .
    \item Sample an edge inside \(G_\dimm(M)\).
\end{enumerate}
\medskip

% When \(\Mgras=\M(\Gr)\) this lemma was proven in \cite[Proposition 55]{Golowich2023}; the proof for arbitrary \(\Y\) is by decomposing \(\Y'_U\) to small parts that are isomorphic to links of \(\Mgras_U\), and reducing to \cite[Proposition 55]{Golowich2023}.

\paragraph{Step II}Showing that \(\SL(\Y,U)\) is an expander.
\begin{lemma} \label{lem:loc-to-glob-decomp-of-link}
There exists a constant \(\alpha > 0\) such that the following holds. Let \(\Y\) be a \([\dimlin,n,\degree,\lambdai]\)-poset and let \(U \in \Y'(\dimm)\) where \(\Y'=\M(Y)^{\leq d}\). Then
    \(\lambda(\SL(\Y,U)) \leq (0.61 + \dimlin \lambdai)^{\alpha m}\). %where \(m = \frac{\dimlin}{2^\dimm}\).
    
    In particular, there is an absolute constant \(K_1 >0\) such that the following holds. Let \(\lambdao > 0\). If \(\dimlout \geq K_1 + \log \log \frac{1}{\lambdao}\), \(\dimlin \geq 2^{2\dimlout}\) and \(\lambdai \leq \frac{1}{4\dimlin}\), then
    \[\lambda(\SL(\Y,U)) \leq \lambdao.\]
\end{lemma}
%We note that \(\dimlin > 2\diml\), and so a priori \(\lambda'\) may depend on \(\dimlin\) but we can always take the \(2\diml+1\)-skeleton of \(\Y\) instead of \(\Y\) itself.

Here is the main place where we use \pref{lem:local-to-global} and the main novelty of our work over \cite{Golowich2023}. As one observes when considering the sampling process underlying  \pref{def:sparsified-link-graph}, one first samples a pair \((w_1,w_2) \in \Y_{w_R}(\dimlin)\times \Y_{w_C}(\dimlin)\) \snote{$\dimlin$ or $m$?} \Ynote{should be top dimension}. Then one samples an edge in \(\SL(\Gr(w_1),\Gr(w_2),U)\), the subgraph induced by \emph{all} rank \(\frac{m}{2}\) matrices whose row and column spaces sit inside \(w_1\) and \(w_2\) respectively. %\snote{is this really an induced subgraph? It doesn't contain all edges among the vertices?}\Ynote{yes. This is because all subspaces in \(w_1\) (resp. \(w_2\)) must also be in \(\Y\).}.
This suggests a local decomposition of \(\SL(\Y,U)\), where our local subgraphs are the subgraphs induced by a fixed pair \((w_1,w_2)\). We analyze the expansion of \(\SL(\Gr(w_1),\Gr(w_2),U)\) in \pref{sec:complete-graph-analysis}. One must also analyze the local-to-global graph \(\B_\tau\) in order to use \pref{lem:local-to-global} (see \pref{sec:local-to-global}). In this case, \(\B_\tau\) itself can be decomposed to a tensor \(G\otimes G\otimes K\) where \(K\) is a complete bipartite graph, and \(G\) is a containment graph of \(\Y\) as defined in \pref{sec:prelims-Grassmann}. This containment graph is an excellent expander when \(\Y\) is \(\lambdai\)-expanding.

% \paragraph{Step III}Showing that \(G_\dimm\) is an expander:
% \begin{lemma} \label{lem:complete-part-analysis} There exists \(\alpha > 0\) such that
%     \(\lambda(G_\dimm) \leq 2^{-\alpha m}\) where \(m=\frac{\dimlin}{2^\ell}\). In particular there is an absolute constant \(K_2 >0\) such that the following holds. Let \(\lambdao > 0\). If \(\dimlout \geq K_2 + \log \log \frac{1}{\lambdao}\) and \(\dimlin \geq 2^{2\dimlout}\) then
%     \[\lambda(G_\dimm) \leq \lambdao\]
%     for every \(\dimm \leq \dimlout\).
% \end{lemma}
% This part is independent of any \(\Y\) and is mostly arguments about matrices. We apply \pref{lem:local-to-global} to reduce the expansion of $G_\dimm$ to the expansion of a related graph \(G_{m'}^0\). The matrices in \(G_{m'}^0(M)\) are rank \(\frac{m}{3}\) matrices \(A \leq M\) and \(A_1,A_2\) are connected if there is a decomposition of \(M\) where \(A_1\) and \(A_2\) are ``disjoint'' parts of the decomposition, i.e.
% \begin{enumerate}
%     \item \(M = \sum_{j=1}^{m} e_j \otimes f_j\).
%     \item \(A_1 = \sum_{j=1}^{\frac{m}{3}} e_j \otimes f_j\) and \(A_2 = \sum_{j=\frac{m}{3}+1}^{\frac{2m}{3}} e_j \otimes f_j\).
% \end{enumerate}
% This graph can now be analyzed by induction. To analyze it, we actually take the ranks of the matrices \(A \leq M\) to be a parameter \(a\) instead of \(\frac{m}{3}\), and bound the expansion of these graphs by induction on \(a\). The base case where \(a=1\) just follows from the fact that the walk is close to uniform in \(TV\)-distance (\pref{claim:base-case}). The inductive step also uses a local-to-global argument a la \pref{lem:local-to-global} (\pref{claim:bound-on-disjoint-bipartite-graph}).

% Although \cite{Golowich2023} has similar statements about expansion of such graphs, the analysis in \cite{Golowich2023} uses arguments that depend on field size which we cannot use. Therefore our proofs are different.

Given these three components the proof for \pref{thm:one-step-of-recursion} is immediate.
\begin{proof}[Proof of \pref{thm:one-step-of-recursion}]
    Let us verify all parameters \([\dimlout,n^2,\dimlin \degree, \lambdao]\). The dimension \(\dimlout\) is clear from the construction. 
    
    The size \(|\Y'(1)| \leq |\Y(1)|^{2 \cdot \frac{\dimlin}{2}}\) since it is enough to specify \(\dimlin\) vectors to construct a rank \(\frac{\dimlin}{2}\) matrix \(M = \sum_{j=1}^{\frac{\dimlin}{2}} e_j \otimes f_j\) (of course we have also double counted since many decompositions correspond to the same matrix). Thus \(\log |\Y'(1)| \leq \dimlin \cdot D \).

    Let us verify that the ambient space is \(n^2\) dimensional, or in other words that \(\Y'(1)\) really spans all \(n \times n\) matrices (recall that we assumed without loss of generality that \(\Y\)'s ambient space is \(\mathbb{F}_2^n\)). For this it is enough to show that there are \(n^2\) linearly independent matrices inside \(\Y'(1)\). Let \(e_1,e_2\dots,e_n \in \Y(1)\) be \(n\) linearly independent vectors. The ambient space of \(Y\) is \(\F_2^n\). Let us show that \(e_i \otimes e_j\) is spanned by the matrices inside \(\Y'(1)\). Indeed, choose some subspaces \(w_i,w_j \in \Y(\dimlin)\) such that \(e_i \in w_i, e_j \in w_j\). Then $\Y'(1)$ contains all rank \(\frac{\dimlin}{2}\) matrices in $\F_2^{n^2}$ whose row and column spans are inside \(w_i,w_j\). These matrices span all matrices whose row and column spans are in \(w_i,w_j\) and in particularly they span \(e_i \otimes e_j\). 
       
    Finally let us show that all links are \(\lambdao\)-expanders. Fix \(U \in \Y' (\dimm)\). By \pref{lem:grassmannian-link-decomposition}
    \[\Y'_U \cong G_\dimm^{\otimes 2^{\dimm}-1} \otimes \SL(\Y,U)\]
    so \(\lambda(\Y'_U) \leq \max \set{\lambda(G_\dimm), \lambda(\SL(\Y,U))}\).
    Both are expanders by \pref{lem:complete-part-analysis} and \pref{lem:loc-to-glob-decomp-of-link}.

    To sum up, \(\Y'\) is a \([\dimlout,n^2,\dimlin \cdot \degree, \lambdao]\)-expanding poset.
\end{proof}
\begin{remark}
    For the readers who are familiar with \cite{Golowich2023}, we remark that contrary to that paper, we do not use the strong trickling down machinery developed in \cite{kaufmanT2021garland}. \cite{kaufmanT2021garland} show that expansion in the top-dimensional links trickles down to the links of lower dimension (with a worse constant, but still sufficient for our theorem). A priori, one may think that using \cite{kaufmanT2021garland} could simplify the proof. However, in our poset all links have the same abstract structure, so we might as well analyze all dimensions at once. Moreover, one observes that in many cases the bound on the expansion of these posets actually \emph{improves} when considering lower dimensions.
\end{remark}


==> Yotam_s_drafts/old/old_sec_7.tex <==


%In \pref{sec:construction-subpoly-HDX} and \pref{sec:spectral-Johnson}, this structure is used to analyze the spectral expansion of these links.

%\paragraph{Johnson Grassmann poset}For two sets \(A,A'\) of the same size \(n > 0\), the graphs \(J(A,k,\ell) \cong J(A,k,\ell)\), so when we do not care about the specific set, we write \(J(n,k,\ell)\).
% \begin{lemma}[Johnson Grassmann poset] \label{lem:links-of-Johnson}
%     Fix \(d\) and \(n\) and let \(Y=Y^{\mathcal{S}_J}\). Let \(1 \leq i \leq d-2\) and let \(W \in Y(i)\). Then the link graph
%     \[\bar{Y}_W \cong J^{\otimes 2^i -1} \otimes J'\]
%     where \(J=J(2^{d-i},2^{d-i-1},2^{d-i-2})\) and \(J' = J(n-2^d+2^i,2^{d-i-1},2^{d-i-2})\) are Johnson graphs.
% \end{lemma}

% Let \(m > 0\) and let \(M \in \MP(4m)\). Denote by  \(\under^M\) the graph that is double covered by \(\mathcal{S}^M(2m,m)\) as in \pref{def:upper-bounded-sum-graph}. That is, the graph whose vertices are \(\MP^M(2m) = \sett{A \in \MP(2m)}{A \leq M}\) and whose edges are all pairs \(A,B\) such that there exists some \(C \in \MP^M(m)\) such that \(C \oplus (A-C) \oplus (A-B) \leq M\). For every two \(M_1,M_2 \in \MP(4m)\) the graphs \(\under^{M_1} \cong \under^{M_2}\), so when we don't care about the matrix \(M\) itself, we write \(\under^{m}\) instead of \(\under^M\).
%
% Similarly, for \(i,m > 0\) and \(M \in \MP(i)\) we define \(\disjointgraph_{M,m}\) to be the graph covered by \(\mathcal{S}_{\cap M}(2m,2m,m)\). That is, the vertices are \(\MP_{\cap M}(m) = \sett{A \in \MP(i)}{A \oplus M}\). We connect \(A,B\) if there exists \(C \in \MP_{\cap M}(m)\) such that \(M \oplus C \oplus (A-C) \oplus (B-C)\). Here we write \(\disjointgraph_{i,m}\) when we don't care about \(M\) itself, only on its rank.
%Let us restate \pref{prop:louis-decomposition} by \cite{Golowich2023}. 

% Recall the definitions of \(\under^m\) and \(\disjointgraph_{i,m}\) in \pref{sec:construction-subpoly-HDX}. %The following lemma (and the main components from the proof we give) was essentially proven in \cite[Proposition 55]{Golowich2023}, albeit in different terminology. 
% %
% \begin{lemma}[Matrix Grassmann poset, restatement of {\pref{prop:louis-decomposition}}] \label{lem:links-of-Grassmann}
%     Fix \(d\) and \(n\). Let \(1 \leq i \leq d-2\) and let \(W \in Y^{\mathcal{S}_{\MP}}(i)\). Set \(m = 2^{d-i-2}\). Then the link graph
%     \[\bar{Y}^{\mathcal{S}_{\MP}}_W \cong (\under^m)^{\otimes 2^i - 1} \otimes \disjointgraph_{2^d-2^i,m}\]
% \end{lemma}

% \paragraph{Sparsified Matrix Grassmann poset} the sparsification has a tensor decomposition that is quite similar to that of \(Y^{\mathcal{S}_{\MP}}\). The components \(\under^m\) remain unmodified, but we replace \(\disjointgraph_{n-2^d+2^i,m}\) with the following graph.
% \begin{definition}[Sparsified link graph] \label{def:sparsified-link-graph}
%    Let \(w \in Y^{\mathcal{S}_{Y_0}}(i)\) and let \(M_w\) be a matrix whose rowspan is \(\sum_{A \in w}row(A)\) and whose colspan is \(\sum_{A \in w}col(A)\).\footnote{The definition does not depend on the matrix \(M_w\), only on its row and column spans.} Set \(m=2^{d-i-1}\). The graph \(\SL(Y_0,w)\) is the graph with vertex set
%     \[ V = \sett{A \in \MP_{\cap M_w}(2m)}{\row(A) \oplus \row(M_w), \; \col(A) \oplus \col(M_w)  \in Y_0 \left(2^d-2^i \right)}.\]
%     The edges are all \(A_1,A_2\) such that there exists a matrix \(B \in \MP_{\cap M_w}(4m)\) such that \(\row(B) \oplus \row(M_w), \; \col(B) \oplus \col(M_w) \in Y_0\), and \(\set{A_1, A_2}\) are an edge in \(\under^M\).
% %
% % Moreover, we also denote \(L(\Y_1,\Y_2,U)\) the same graph as above with the distinction that we require \(\row(A) \oplus \row(S_U) \in \Y_1\) and \(\col(A) \oplus \col(S_U)  \in \Y_2\) (and similarly for the edges).
% \end{definition}

% \begin{lemma} \label{lem:links-of-sparsemann}
%     Fix \(d\) and \(n\). Let \(Y_0\) be a \(2^d-1\)-dimensional Grassmann poset. Let \(Y=Y^{\mathcal{S}_{Y_0}}\). Let \(1 \leq i \leq d-2\) and let \(w \in Y(i)\). Set \(m = 2^{d-i-2}\). Then the link graph
%     \[\bar{Y}_w \cong (\under^m)^{\otimes 2^i - 1} \otimes \SL(Y_0,w)\]
% \end{lemma}
% We comment that formally, the distribution over edges in the sparsified link graph \(\SL(\Y,w)\) is the following. %Let \(w_R = \row(S_U)\) and \(w_C = \col(S_U)\):
%  \begin{enumerate}
%      \item Sample \(w_1 \in Y_{\row(M_w)}(2^d-1)\) and \(w_2 \in Y_{\col(M_w)}(2^d-1)\) according to the respective distributions of \(Y_{\row(M_w)}(2^d-1),Y_{\col(M_w)}(2^d-1) \).
%      \item Uniformly sample a matrix \(M\) %of rank \(4m\) 
%      such that \(\row(M_w) \oplus \row(M) = w_1\) and \(\col(M_w) \oplus \col(M) = w_2\) .
%      \item Sample an edge in \(\under^M\).
%  \end{enumerate}

%The remainder of this section is dedicated to proving these two lemmas, but before doing so we take a detour to give a description of the lower dimensional skeletons of \(Y^{\mathcal{S}}\) that we will use when analyzing the link structure.

% \subsubsection[Structure of links of the Johnson]{Structure of links of \(Y^{\mathcal{S}_J}\) - examples of low dimensional links}
% Using the previous observation on the induced structure of lower dimensional subspaces, we take this one step further and illuminate the structure of the links in the induced Grassmann posets. It turns out that in the examples above, links are tensor products of simpler graphs. This was already observed by \cite{Golowich2023} in the matrix case. However, we start with the simpler Johnson Grassmann case. %While we do not formalize an abstract theorem on when this phenomenon occurs, we discuss possible abstractions in the end of this section.

% Before proving \pref{lem:links-of-Johnson}, let us give two examples for intuition: the link of \(\set{0}\) (i.e.\ the entire poset) and a link of a \(1\)-dimensional subspace.  Recall that we identify vectors \(w \in \F_2^n\) with the set of coordinates \(w \subseteq [n]\) on which the vector \(w\) is equal \(1\).
% \paragraph{The link of \(\set{0}\)} In this case we claim that \(\bar{Y}^{\mathcal{S}_J}_{\set{0}} \cong J' = J(n,2^{d-1},2^{d-2})\). Indeed, the vertices in \(Y^{\mathcal{S}_J}(1)\) are all vectors of weight \(2^{d-1}\). Two vectors \(x,y\) form a \(2\)-dimensional subspace \(\sp (x,y) \in Y^{\mathcal{S}_J}(2)\) if and only if there is a function \(s:\F_2^2 \to \F_2^n\) such that \(|s(1,0)|=|s(0,1)|=|s(1,1)|=2^{d-2}\), their supports are mutually disjoint, and such that
% \begin{equation} \label{eq:xy-example-zero-dimensional}
%     \widehat{s}(1,0) = w_1 =s(1,0) + s(1,1), \; \ve ; \widehat{s}(0,1) = w_2 =s(0,1) + s(1,1).
% \end{equation}
% Here we are using the fact that the two dimensional subspaces are given by \(\mathcal{S}_2\) as described in \pref{ex:johnson-subspaces}.

% The fact that the supports of every pair of \(s(i,j)\) and \(s(i',j')\) are mutually disjoint shows that the coordinates in \(x \cap y\) are exactly \(s(1,1)\), i.e.\ they intersect on half their coordinates. Thus if \(w_1\) and \(w_2\) are connected by an edge in the link graph of \(\set{0}\), then they are connected by an edge in \(J(n,2^{d-1},2^{d-2})\). Conversely, if \(w_1\) and \(w_2\) that are connected in the Johnson, one can define \(s \in \mathcal{S}_2\) that satisfies \eqref{eq:xy-example-zero-dimensional} by setting \(s(1,0) = w_1 \setminus w_2\), \(s(1,1) = w_1 \cap w_2\) and \(s(0,1) = w_2 \setminus w_1\). This implies that \(\sp(w_1,w_2) \in Y^{\mathcal{S}_J}(2)\).

% \paragraph{A one-dimensional subspace's link}Let \(w \in Y^{\mathcal{S}_J}(1)\). We introduce the following notation: for a finite set \(A\) we write \(J(A,k,\ell)\), as a Johnson graph whose vertices are subsets \(t \subseteq A\) of size \(k\) and two subsets \(t_1,t_2\) are connected if \(|t_1 \cap t_2| = \ell\). With this notation we will see that \(\bar{Y}^{\mathcal{S}_J}_w \cong J \otimes J'\) where \(J = J(w,2^{d-2},2^{d-3})\) and \(J' = J([n] \setminus w,2^{d-2},2^{d-3})\).

% Indeed, in the first example we saw that we can decompose every \(y \in Y^{\mathcal{S}_J}_w(1)\) to \(y=y_1 + y_2\) where \(y_1 \subseteq w\), \(y_2 \cap w = \emptyset\) and both \(|y_1|=|y_2|=2^{d-2}\).

% The isomorphism \(\psi\) between \(Y^{\mathcal{S}_J}_w \cong J \otimes J'\) maps \(y \overset{\psi}{\mapsto} (y_1,y_2)\). By definition \(y_1 \subseteq w\) is a vertex in \(J\) and \(y_2\) is a vertex in \(J'\) because \(y \cap w = \emptyset\). Let \(y,y'\) be a pair of vertices in \(Y_w^{\mathcal{S}_J}\) that are mapped to \(\psi(y)=(y_1,y_2), \psi(y')=(y_1',y_2')\). Let us argue that \(\set{y,y'}\) is an edge in the link of \(w\) if and only if \(y_1 \sim y_1'\) and \(y_2 \sim y_2'\) in the respective Johnson graphs \(J\) and \(J'\). 

% First, let us assume that \(\set{y,y'}\) is an edge in the link of \(w\), that is, \(\sp(w,y,y') \in Y^{\mathcal{S}_J}(3)\). We take some \(s \in \mathcal{S}_3\) such that \(Im(\widehat{s}) = \sp(w,y,y')\). Note that \(\mathcal{S}_3\) is closed under composition with \(GL_3(\F_2)\)\footnote{that is, \(s \circ g \in \mathcal{S}_3\) for any \(s \in \mathcal{S}_3\) and \(g \in GL_3(\F_2)\).}, so we can assume without loss of generality that
% \[\widehat{s}(1,0,0)= w = \sum_{v:\iprod{(1,0,0),v}=1}s(v) = \sum_{b_1,b_2 \in \set{0,1}}s(1,b_1,b_2)\]
% and similarly
% \[\widehat{s}(0,1,0)= y = \sum_{b_1,b_2 \in \set{0,1}}s(b_1,1,b_2)\]
% and
% \[\widehat{s}(0,0,1)= y' = \sum_{b_1,b_2 \in \set{0,1}}s(b_1,b_2,1).\]
% We observe that \(y_1 = y \cap w = s(1,1,0)+s(1,1,1)\) and similarly that \(y_1' = s(1,0,1)+s(1,1,1)\) so the intersection \(y_1 \cap y_1' = s(1,1,1)\) is of size \(2^{d-3}\) (since this is the weight of every element in the image of \(s\)). Similarly, one can calculate that \(|y_2 \cap y_2'| = |s(0,1,1)|=2^{d-3}\). Thus \(y_1 \sim y_1'\) and \(y_2 \sim y_2'\) in the respective Johnson graphs.

% Conversely, given \((y_1,y_2) \sim (y_1',y_2')\) in the tensor product, one can reconstruct \(s \in \mathcal{S}_3\) so that \(Im(\widehat{s})=\sp(w,x,y)\). With the notation \(a^b = \begin{cases}
%     a & b=1 \\
%     [n] \setminus a & b=0
% \end{cases}\) for \(a \in \F_2^n\), we set \(s(i,j,k)=w^i \cap y^j \cap y'^k\). One can verify that \(s \in \mathcal{S}_3\) and that \(Im(\widehat{s})=\sp(w,y,y')\).

% \subsubsection[Overview of the proof of the decomposition lemma of the Johnson]{Overview of the proof of the decomposition lemma of \(Y^{\mathcal{S}_J}\)}
% Unfortunately, moving to links of higher dimensional subspaces soon becomes intractable. However, we can already conclude that given an edge \(\set{y,y'}\) in the link, we need to construct a function \(s\) such that its values \(s(x)\) correspond to intersections of \(y,y'\) and vectors in \(W\). Let us draw our strategy in more detail.

% Fix \(i \geq 1\) and a subspace \(W \in Y^{\mathcal{S}_J}(i)\),
% \begin{enumerate}
%     \item We argue that even though there could be many \emph{different} \(s \in \mathcal{S}_J\) so that \(W=Im(\widehat{s})\), the set \(Im(s)\) is uniquely determined. We denote this set \(Q_W\). More precisely, \(z \in Q_W\) if and only if there is a co-dimension \(1\) affine subspace \(W' \subseteq W\) such that \(z = \bigcap_{y \in W'}y\).
%     \begin{claim} \label{claim:uniqueness-of-s-pieces}
%         Let \(W \in \Y^{\mathcal{S}_J}(i)\). Then for every \(s_V,s'_{V'} \in \mathcal{S}_i\) such that \(W=Im(\widehat{s_V})=Im(\widehat{s'_{V'}})\) the sets \(\sett{s_V(v+V)}{v+V \ne 0+V}\) and \(\sett{s'_{V'}(v+V')}{v+V' \ne 0+V'}\) are equal. We denote this set \(Q_W\). 
%     \end{claim}
%     \item Based on \(Q_W\), we give the following criterion for being in the link of \(W\). 
%     \begin{claim} \label{claim:johnson-link-criterion}
%         Fix \(W \in Y^{\mathcal{S}_J}(i)\) and let \(Q_W = \set{z_j}_{j=1}^{2^i - 1}\). Then \(y \in Y^{\mathcal{S}_J}_W(1)\) if and only if there exists \(y_1,y_2,\dots,y_{2^i}\) of weight \(2^{d-i-1}\) such that \(y = \sum_{j=1}^{2^i} y_j\), for \(j\leq 2^i -1\), \(y_j \subseteq z_j\) and \(y_{2^i}\) is disjoint from all the \(z_j\)'s.
%         %
%         Moreover, with \(W' = W + \sp (y)\), \(Q_{W'} = \set{y_j}_{j=1}^{2^i} \cup \set{z_j-y_j}_{j=1}^{2^i - 1}\).
%     \end{claim}
%     \item We use \pref{claim:johnson-link-criterion} to define the map \(\psi: Y^{\mathcal{S}_J}_W \to \left ( \bigotimes_{j=1}^{2^i-1} J_j  \right ) \otimes J'\) where 
%     \[J_j = J(z_j,2^{d-i-1},2^{d-i-2})\]
%     and
%     \[J' = J([n] \setminus \bigcup_{j=1}^{2^i-1} z_j,2^{d-i-1},2^{d-i-2}).\]
%     The map takes \(y\) and maps it to \((y_1,y_2,\dots,y_{2^i})\) where \(y_j \subseteq z_j\) for \(j \leq 2^i -1\) and \(y_{2^i}\) is disjoint from all the \(z_j\)'s. As we will see below, if will follow from \pref{claim:johnson-link-criterion} that this map is well defined, and it is the desired isomorphism.
% \end{enumerate}

% Let us prove the two auxiliary claims and then continue to the proof of \pref{lem:links-of-Johnson}.
% \begin{proof}[Proof of \pref{claim:uniqueness-of-s-pieces}]
%     Let us assume that \(V=V'\) for simplicity (but the two maps \(s\) and \(s'\) are not necessarily the same). This is without loss of generality since we can always compose \(s'\) with an invertible linear operator that maps \(V^{\bot}\) to \(V'^{\bot}\), which will not change \(W\). We also denote \(U = V^\bot\).

%     We now prove that \(s_V(v+V)\) is given by the formula
%     \begin{equation} \label{eq:formula-for-sets}
%         s_V(v+V) = \bigcap_{x \in U, x \notin \sp(v)^\bot} \widehat{s_a}(x).
%     \end{equation}
%     %Here the intersection is the vector obtained by the entrywise \(AND\) in \(\F_2^n\).
%     Before proving this formula is true, let us explain why the claim follows from it. Every \((i-1)\)-dimensional subspace of \(U\) is given by \(\sp(v)^{\bot} \cap U\) for some \(v+V \in \nicefrac{\F_2^d}{V} \setminus \set{0+V}\) (and \(\sp(v)^{\bot} \cap U = \sp(v')^{\bot} \cap U\) if and only if \(v+V = v'+V\)). Thus the set \(\sett{s_V(v+V)}{v+V \ne V}\) is equal to 
%     \[ \sett{\bigcap_{x \in U \setminus U'} \widehat{s_V}(x)}{U' \subseteq U, \dim(U')=i-1}.\]
%     Writing \(W = Im(\widehat{s_V}) = Im(\widehat{s_{V'}})\) this is also equal to 
%     \[ \sett{\bigcap_{y \in W \setminus W'} y}{W' \subseteq W, \dim(W')=i-1}\]
%     since going over all \(U' \subseteq U\) of dimension \((i-1)\) in the domain is the same as going over all subspaces inside the image, is the same as going over all subspaces of \(W\) of the same dimension. As we can see, this set is independent of \(s_V\) since it has a description depending only on vectors and subspaces of \(W\).

%     It remains to argue that the formula holds. For this we simply observe that the supports of the \(s_V(v+V)\) are mutually disjoint, and the only coordinates that appear in $\widehat{s_V}(x)$ for all \(x \notin v^\bot\) are those of \(s_V(v+V)\).
% \end{proof}

% \begin{proof}[Proof of \pref{claim:johnson-link-criterion}]
%     Fix \(W \in Y^{\mathcal{S}_J}(i)\) and let \(y \in \bar{Y}^{\mathcal{S}_J}_W(1)\) and denote by \(W' = W + \sp(y)\). Let \(s:\F_2^d \to \F_2^n\) be such that \(W'=\widehat{s}|_{U'}\) and \(W=\widehat{s}|_{U}\) for a pair of \(i\) and \((i+1)\)-dimensional spaces \(U \subseteq U'\). We write \(V=\sp \set{b_1,b_2,\dots,b_{d-i}}\) and \(V'=\set{b_1,b_2,\dots,b_{d-i-1}}\) such that \(U'=V'^{\bot}, U=V^\bot\). Then every \(v+V \in \nicefrac{\F_2^d}{V}\) can be partitioned into two cosets of \(V'\), namely, \(v+V = v+V' \dunion (v+b_{d-i})+V'\). Moreover, by definition,
%     \[s_V(v_0+V) = \sum_{v' \in v_0+V}s(v) = \sum_{v' \in v+V'}s(v') + \sum_{v' \in (v_0+b_{d-i})+V'}s(v') = s_{V'}(v_0+V') + s_{V'}((v_0+b_{d-i})+V').\]
%     Let \(x \in U' \setminus U\) be such that \(\widehat{s}(x)=y\); we saw in \pref{claim:skeleton-of-induced-Grassmann} that \(\widehat{s_{V'}}(x)=y\) also. As \(e \in U' \setminus U\), \(\iprod{e,b_{d-i}} = 1\) and therefore, \(\iprod{x,v+V'} \ne \iprod{e,(v+b_{d-i})+V'}\). This implies that that for every \(v_0+V \ne V\), \(y \cap s_V(v_0+V)\) is one of \(s_{V'}(v_0+V'), s_{V'}((v_0+b_{d-i})+V')\) --- and therefore we will be able to define one of the \(y_j = y \cap s_V(v_0+V)\) inside \(z_j = s_V(v_0+V)\). Indeed:
%     \begin{align*}
%         \widehat{s_{V'}}(x) &= \left (\sum_{v+V' \not\subseteq v_0+V} \iprod{x,v+V'}s_{V'}(v+V') \right )\\
%     &+  \left ( \iprod{x,v_0+V'}s_{V'}(v_0+V') + \iprod{x,(v_0+b_{d-i})+V'}s_{V'}(v_0+V') \right ).
%     \end{align*}
% The sum in the first line contributes nothing to \(s_V(v_0+V) \cap y\) since every \(s_{V'}(v+V')\) has an empty intersection \(s_V(v_0+V)\) when \(v+V' \not\subseteq v_0+V\). Among the final two terms of the sum, exactly one of the inner products is non-zero, proving that \(y \cap s_V(v_0+V)\) is one of \(s_{V'}(v_0+V'), s_{V'}((v_0+b_{d-i})+V')\).

% Thus we index \(z_j = s_V(v+V)\) (arbitrarily) and set \(y_j = z_j \cap y\). We also set \(y_{2^i} = s_{V'}(b_{d-i})\) and note that \(y_{2^i}\) also participates in the linear combination of \(\widehat{s_{y'}}(x)\) because \(\iprod{x,b_{d-i}}=1\). All \(y_j\)'s have weight \(2^{d-i-1}\) and by the discussion above, we have that \(y = \sum_{j=1}^{2^i} y_j\). Moreover, \(y_j \subseteq z_j\) for every \(j \leq 2^i-1\) and \(y_{2^i}\) is disjoint from all \(z_j = s_V(v+V)\). Finally, we note that \(Q_{W'} = \sett{s_{V'}(v+V')}{v+V' \ne V'} = \set{y_j}_{j=1}^{2^i} \cup \set{z_j-y_j}_{j=1}^{2^i - 1}\) by construction.

% Let us prove the converse -  that if \(y\) satisfies the criterion in the claim, then \(y\) is in \(W\)'s link. Given \(W\) and the \(y_j\)'s let us construct some \(s' \in (\mathcal{S}_J)_{i+1}\) with \(Im(\widehat{s})=W + \sp(y)\). Let \(s \in \mathcal{S}_i\) be such that \(Im(s) = W\) and without loss of generality \(s:\F_2^i \to \F_2^n\), and re-index the \(y_{j}\)'s such that \(y_{v} \subseteq s(v)\) for every \(v \ne 0\) (and keep \(y_{2^i}\) to be the part disjoint from every \(s(v)\)). Set \(s':\F_2^{i+1} \to \F_2^n\) to be as follows. For input \((b,v) \in \F_2 \times \F_2^{i}\),
% \[s'(b,v) = \begin{cases}
%     y_v + (1-b)s(v) & v \ne 0\\
%     y_{2^i} & (b,v)=(1,\bar{0})
% \end{cases}.\]
% It is easy to observe that \(\widehat{s'}(1,\bar{0}) = \sum_{v \in \F_2^i}s'(1,v) = y_{2^i} + \sum_{v_\in \F_2^{i} \setminus 0} y_v = y\). Moreover, we claim that for \(U'' = \sett{(0,v)}{v \in \F_2^i}\), \(Im(\widehat{s'}|_{U''}) = w\). This follows because 
% \[\widehat{s'}(0,v) = \sum_{(b,v') \in \F_2^{i+1} \setminus \{0\}}\iprod{(b,v'),(0,v)}s'(b,v') = \sum_{v' \in \F_2^{i} \setminus \{0\}}\iprod{v',v}(s'(0,v')+s'(1,v')) = \widehat{s}(v).\]
% The second equality is because \(s'(0,v')+s'(1,v') = s(v)\). Therefore \(Im(\widehat{s'}) = W + \sp(y)\) and \(y\) is in the link of \(W\) as required.
% \end{proof}

% \begin{proof}[Proof of \pref{lem:links-of-Johnson}]   
%     Let \(Q_W = \set{z_j}_{j=1}^{2^i-1}\). We will show that \(\bar{Y}^{\mathcal{S}_J}_W \cong \left (\bigotimes_j J(z_j,2^{d-i-1},2^{d-i-2}) \right ) \otimes J([n] \setminus \left (\bigcup_{j=1}^{2^i-1}z_j \right ),2^{d-i-1},2^{d-i-2}) \coloneqq \mathcal{J}\).
%     We define a map \(\psi: Y^{\mathcal{S}_J}_w(1) \to \mathcal{J}\) sending \(y \mapsto (y_1,y_2,\dots,y_{2^i})\) where the \(y_j\)'s are as in \pref{claim:johnson-link-criterion}. By \pref{claim:johnson-link-criterion} this map is well defined for every \(y\) and sends link vertices into vertices of \(\mathcal{J}\). Obviously it is injective, since the disjoint union of the \(y_j\)'s is \(y\). Moreover, by the other direction of \pref{claim:johnson-link-criterion} this is also a bijection, that is, \(\psi^{-1}(y_1,y_2,\dots,y_{2^i})=\sum_{j=1}^{2^i} y_j \in \bar{Y}^{\mathcal{S}_J}_{W}(1)\).

%     We prove that \(\psi\) is a graph isomorphism. A pair \(\set{y,y'}\) is an edge in \(\bar{Y}^{\mathcal{S}_J}_W\) if and only if \(y \in \bar{Y}^{\mathcal{S}_J}_{W'}(1)\) where \(W'=W+\sp(y)\).
%     Applying \pref{claim:johnson-link-criterion} to \(W\) and \(y\), we get \(Q_{W'} = \set{y_j} \cup \set{z_j - y_j}\). Applying \pref{claim:johnson-link-criterion} to \(W'\) we have that \(y' \in \bar{Y}^{\mathcal{S}_\MP}_{W'}(1)\) if and only if we can decompose \(y'=\sum_{j=1}^{2^{i+1}}y_j'\) such that \(y_{2^{i+1}}\) is disjoint from (the supports of) the vectors \(Q_{W'}\), and for every \(j < 2^{i+1}\) there is a distinct vector \(t_j \in Q_{W'}\) such that \(y_j' \subseteq t_j\). Let us re-index the \(y_j'\)'s and \(t_j'\)'s with \[t_{j,b} = \begin{cases}
%         y_j & b=0 \\ z_j - y_j & b=1
%     \end{cases}.\]
%     So on the one hand, if \(\psi(y),\psi(y')\) are neighbors, we can take \(y_{j,0}' = \psi(y')_j \cap \psi(y)_j\) and \(y_{j,1}' = \psi(y')_j \setminus \psi(y)_j\) which will satisfy criterion in \pref{claim:johnson-link-criterion}, and therefore prove that \(y,y'\) are neighbors in the link.
    
%     For the converse direction, if there exists such a decomposition of \(y'\) then it is straightforward to verify that \(y_j'  =y_{j,0}' + y_{j,1}'\), so \(y_j'\) intersects \(y_j\) on half the vertices, or in other words, they are edges in the corresponding Johnson graphs. Thus \(\set{\psi(y),\psi(y')} \in \mathcal{J}\).
% \end{proof}

% \subsubsection{The Decomposition Lemma for the Matrix Induced Grassmann}
% We move on to prove the analogous claim for the matrix Grassmann. Our proof follows the same paradigm as in the Johnson case: we start by showing that the image of every \(s\) such that \(W=Im(\widehat{s})\) is the same \pref{claim:uniqueness-of-s-pieces}; then we give a criterion based on the set in \pref{claim:uniqueness-of-s-pieces} for a matrix being in the link, similar to \pref{claim:johnson-link-criterion}. Finally, we use this criterion to prove the decomposition lemma. 

% We start with a claim similar to \pref{claim:uniqueness-of-s-pieces}, for the matrix case. 
% \begin{claim} \label{claim:uniquness-of-matrix-pieces}
%     Let \(W \in \Y^{\mathcal{S}_{\MP}}(i)\). Then for every \(s_V,s'_{V'} \in \mathcal{S}_i\) such that \(W=Im(\widehat{s_V})=Im(\widehat{s'_{V'}})\) the sets \(\sett{s_V(v+V)}{v+V \ne V}\) and \(\sett{s'_{V'}(v+V')}{v+V'\ne V'}\) are equal. 
% \end{claim}
% We denote the set \(\sett{s_V(v+V)}{v+V \ne V}\) by \(Q_W\).

% This time we replace the intersection in the Johnson case, with a matrix \(GCD\) as defined by the following claim.
% \begin{claim} \label{claim:containment-in-shared-matrix}
%     Let \(A,B \leq C\) be such that \(\row(A) \subseteq \row(B)\) and \(\col(A) \subseteq \col(B)\). Then \(A \leq B\).

%     In particular, if for a set of matrices \(\set{C_i}_{i \in I}\) there exists a matrix \(B\) such that for every \(i\in I\), \(B \leq C_i\) and \(\row(B) = \bigcap_{i \in I} \row(C_i)\), \(\col(B) = \bigcap_{i \in I} \col(C_i)\). 
%     %
%     Then \( \forall i \in I, A \leq C_i\) implies \(A \leq B\).
% \end{claim}
% This claim essentially abstracts the observation in \cite[Lemma 57]{Golowich2023}.

% We notice that if such a \(B\) exists for a set \(\set{C_i}_{i \in I}\), then it is unique. We denote \(B = GCD(\set{C_i}_{i \in I})\) when it exists.

% \begin{proof}[Proof of \pref{claim:containment-in-shared-matrix}]
%     Observe that \(\row(B-A) \subseteq \row(B)\) and \(\col(B-A) \subseteq \col(B)\). Moreover, \((C-B) \oplus B\) which means that \(\row(C-B)\) and \(\col(C-B)\) intersects trivially with \(\row(B)\) and \(\col(B)\) respectively. Thus \((C-B) \oplus (B-A)\). So we get
%     \[ \rank(C-A) = \rank((C-B) + (B-A)) = \rank(C-B) + \rank(B-A).\]
%     On the other hand, because \(A,B \leq C\) this translates to
%     \[\rank(C) - \rank(A) = \rank(C) - \rank(B) + \rank(B-A)\]
%     or equivalently \(\rank(B) = \rank(A) + \rank(B-A)\) i.e.\ \(A \leq B\).

%     As for the `in particular' part. Note that if \(\forall i \in I, A \leq C_i\) then \(\row(A) \subseteq \bigcap_{i \in I} \row(C_i) = \row(B)\) and similarly for the column space. Thus \(A,B \leq C_1\), \(\row(A) \subseteq \row(B), \col(A) \subseteq \col(B)\) and from what we proved \(A \leq B\).
% \end{proof}

% \begin{proof}[Proof of \pref{claim:uniquness-of-matrix-pieces}]
%     The proof follows the same lines as the proof of \pref{claim:uniqueness-of-s-pieces}. Let \(V=V',s,s'\) and \(U\) as in \pref{claim:uniqueness-of-s-pieces}. This time, we note that
%     \[s_V(v+V) = GCD(\sett{\widehat{s_V}(x)}{x \in U, x\notin \sp(v)^\bot}).\]
%     To show this equality we use \pref{claim:containment-in-shared-matrix}. Indeed, \(s_V(v+V) \leq \widehat{s_V}(x)\) whenever \(s_V(v+V)\) appears in the sum that defines \(\widehat{s_V}(x)\), since this sum is direct. This occurs whenever \(x \in U, x\notin \sp(v)^\bot\). Therefore, it suffices to show that the row space (and column space) of \(s_V(v+V)\) is equal to the intersection of row spaces (and column spaces) of the set in the righthand side of the equation.  Let us do the row spaces case: \(\row(s_V(v+V)) = \bigcap_{x \in U, x\notin \sp(v)^\bot} \row(\widehat{s_V}(x))\). Indeed, the fact that \(s_V(v+V) \leq \widehat{s_V}(x)\) implies that \(\row(s_V(v+V)) \subseteq \bigcap_{x \in U, x\notin \sp(v)^\bot} \row(\widehat{s_V}(x))\) so we prove the converse containment.
    
%     For every \(y\) in the intersection of row spaces, and every \(x \in U \cap \sp(v)^{\bot}\), we can uniquely decompose sum \(y=\sum_{u'+V} y_{u'+V}^x\) where we are summing over all \(u'+V\) that appear in the sum defining \(\widehat{s}_V(x)\) and \(y_{u'+V}^x \in \row(s_V(u'+V))\). This decomposition is unique (and exists) because the \(\row(s_V(u'+V))\) are a direct sum of spaces.
    
%     But as \(y\) is in the row span of every \(\widehat{s_V}(x)\) such that \(x \in U, x\notin \sp(v)^\bot\), the only \(y_{u'+V}\)'s that are non-zero are those where the corresponding \(s_V(u'+V)\) appears in the decomposition of \emph{all} the \(\widehat{s_V}(x)\)'s, which is only \(s_V(v+V)\). Thus \(y \in \row(s_V(v+V))\).

%     By the same argument in \pref{claim:uniqueness-of-s-pieces}, the vectors in the image set do not depend on the domain, only on the affine subspaces of the image, and hence the set is unique.
% \end{proof}

% % \iffalse
% % \begin{claim}
% %     Let \(W_1,W_2,\dots,W_n\) be such that \(W_1 \oplus W_2 \oplus ... \oplus W_n\). Let \(I_1,I_2,\dots,I_m \subseteq [n]\) and \(I = \bigcap_{i=1}^m I_i\). Let \(W^{i} = \bigoplus_{j \in I_i} W_j\) and \(W^{\cap} = \bigoplus_{j \in I}W_j\). Then \(W^{\cap} = \bigcap_{i=1}^m W^i\).
% % \end{claim}

% % \begin{proof}
% %     One containment is clear, so we need just to prove that \(W^{\cap} \supset \bigcap_{i=1}^m W^i\). Let \(y \in \bigcap_{i=1}^m W^i\). Let \(y=\sum_{j \in I_1}y_j\) be such that \(y_j \in W_j\). Let us show that for every \(j \notin I\), \(y_j = 0\). Assume not, and assume without loss of generality that \(j \notin I_2\). Let \(y=\sum_{j \in I_2}y_j'\) be such that \(y_j' \in W_j\).
% %     Then we can write
% %     \[\sum_{I_1 \setminus I_2} y_j + \sum_{j \in I_2 \cap I_2} y_j = \sum_{j \in I_2}y_j'\]
% %     or equivalently
% %     \[\sum_{I_1 \setminus I_2} y_j = \sum_{j \in I_2} y_j''\]
% %     where \(y_j'' \in W_j\) are some vectors.
% %     The left hand side is in \(\bigoplus_{j \in I_1 \setminus I_2} W_j\), the right hand side is in \(\bigoplus_{j \in I_2}W_j\). Thus both sides are equal to zero since these two subspaces intersect trivially. In particular, \(\sum_{I_1 \setminus I_2} y_j = 0\) and because the sum \(\bigoplus_{j \in I_1 \setminus I_2} W_j\) is direct then every \(y_j = 0\).
% % \end{proof}
% % \fi
% Next we give our criterion for being in the link of a subspace.
% \begin{claim} \label{claim:characterizing-link-of-w}
%     Let \(W \in Y^{\mathcal{S}_\MP}(i)\) and \(A \in Y^{\mathcal{S}_\MP}(1)\). Denote by \(Q_W=\set{Z_j}_{j=1}^{2^i-1}\) the matrices defining \(W\). Then \(A \in Y^{\mathcal{S}_\MP}_W(1)\) if and only if there exists a decomposition of \(A = \sum_{j=1}^{2^{i}} A_j\) for \(A_j \in \MP(2^{d-i-1})\) where \(A_j \leq Z_j\) for every \(j \leq 2^i -1\) and \(A_{2^i} \oplus \left ( \sum_{j=1}^{2^i - 1} A_j \right )\).
%     %
%     In this case for \(W' = W+\sp(A)\), \(Q_{W'} = \set{A_j}_{j=1}^{2^i} \cup \set{Z_j-A_j}_{j=1}^{2^i-1}\).
% \end{claim}

% \begin{proof}
%     We follow a similar argument as in the proof of \pref{claim:johnson-link-criterion}. 
%     %
%     Fix \(W \in Y^{\mathcal{S}_{\MP}}(i)\) and let \(A \in \bar{Y}^{\mathcal{S}_{\MP}}_W(1)\) and denote by \(W' = W + \sp(A)\). Let \(s:\F_2^d \to \F_2^n\) be such that \(W'=\widehat{s}|_{U'}\) and \(W=\widehat{s}|_{U}\) for a pair of \(i\) and \((i+1)\)-dimensional spaces \(U \subseteq U'\). We write \(V=\sp \set{b_1,b_2,\dots,b_{d-i}}\) and \(V'=\set{b_1,b_2,\dots,b_{d-i-1}}\) such that \(U'=V'^{\bot}, U=V^\bot\). We recall that every \(v+V \in \nicefrac{\F_2^d}{V}\) can be partitioned into two cosets of \(V'\), \(v+V = v+V' \dunion (v+b_{d-i})+V'\) and \(s_V(v+V) = s_{V'}(v+V') + s_{V'}((v+b_{d-i})+V').\)
    
%     Let \(x \in U' \setminus U\) be such that \(\widehat{s}(x)=A\) and as in \pref{claim:skeleton-of-induced-Grassmann}, \(\widehat{s_{V'}}(x)=A\). As before, \(x \in U' \setminus U\), \(\iprod{x,b_{d-i}} = 1\) and therefore, \(\iprod{x,v+V'} \ne \iprod{x,(v+b_{d-i})+V'}\). This implies that that for every \(v_0+V \ne V\), \(GCD(A,s_V(v_0+V))\) is one of \(s_{V'}(v_0+V'), s_{V'}((v_0+b_{d-i})+V')\) (and in particular, exists). Indeed:
%     \begin{align*}
%         A &= \widehat{s_{V'}}(x) = \sum_{v+V' \not\subseteq v_0+V} \iprod{x,v+V'}s_{V'}(v+V') \\
%     &+  \left ( \iprod{x,v_0+V'}s_{V'}(v_0+V') + \iprod{x,(v_0+b_{d-i})+V'}s_{V'}(v_0+V') \right ).
%     \end{align*}
% Assume that \(\iprod{x,v_0+V'}=1\) (the other case is similar). Then \(\row(A) \cap \row(s_V(v_0+V)) = \row(s_{V'}(v_0 +V'))\) and the same holds for the column spaces, therefore by \pref{claim:containment-in-shared-matrix} \(GCD(A,s_V(v+V))=s_{V'}(v_0 +V')\).

% Thus we re-index \(Z_j = s_V(v+V)\) (arbitrarily) and set \(A_j = GCD(Z_j, A)\). We also set \(A_{2^i} = s_{V'}(b_{d-i})\) and note that \(A_{2^i}\) also participates in the linear combination of \(\widehat{s_{V'}}(x)\) because \(\iprod{x,b_{d-i}}=1\). All \(A_j\)'s have rank \(2^{d-i-1}\) and by the discussion above, we have that \(A = \sum_{j=1}^{2^i} A_j\). Moreover, \(A_j \leq Z_j\) for every \(j \leq 2^i-1\) and \(A_{2^i}\) is disjoint from all \(Z_j = s_V(v+V)\). Finally, we note that \(Q_{W'} = \sett{s_{V'}(v+V')}{v+V' \ne V'} = \set{A_j}_{j=1}^{2^i} \cup \set{Z_j-A_j}_{j=1}^{2^i - 1}\) by construction.

% Conversely, fix \(W\) and the \(A_j\)'s and let us construct some \(s' \in (\mathcal{S}_\MP)_{i+1}\) with \(Im(\widehat{s'})=W + \sp(A)\). Let \(s \in \mathcal{S}_i\) be such that \(Im(s) = W\) and without loss of generality \(s:\F_2^i \to \F_2^n\). Re-index the \(A_{j}\)'s such that \(A_{v} \leq s(v)\) for every \(v \ne 0\) (and keep \(A_{2^i}\) to be the part not \(\leq\) any of the \(s(v)\)'s). Set \(s':\F_2^{i+1} \to \F_2^n\) to be as follows. For input \((b,v) \in \F_2 \times \F_2^{i}\),
% \[s'(b,v) = \begin{cases}
%     A_v + (1-b)s(v) & v \ne 0\\
%     A_{2^i} & (b,v)=(1,\bar{0})
% \end{cases}.\]
% It is easy to observe that \(\widehat{s'}(1,\bar{0}) = \sum_{v \in \F_2^i}s'(1,v) = \sum_{j=1}^{2^i} A_j = A\). Moreover, we claim that for \(U'' = \sett{(0,v)}{v \in \F_2^i}\), \(Im(\widehat{s'}|_{U''}) = W\). This follows because 
% \[\widehat{s'}(0,v) = \sum_{(b,v')\in  \F_2^{i+1}\setminus \set{0}}\iprod{(b,v'),(0,v)}s'(b,v') = \sum_{v'\in  \F_2^{i}\setminus \set{0}}\iprod{v',v}(s'(0,v')+s'(1,v')) = \widehat{s}(v).\]
% The second equality is because \(s'(0,v')+s'(1,v') = s(v)\).
% \end{proof}

% \begin{proof}[Proof of \pref{lem:links-of-Grassmann}]
% The proof follows the same lines as \pref{lem:links-of-Johnson}. Let \(Q_W = \set{Z_j}_{j=1}^{2^i-1}\) and write \(Z = \sum_{j=1}^{2^i} Z_j\). We will show that \(\bar{Y}^{\mathcal{S}_\MP}_W \cong \left (\bigotimes_j \under^{Z_j} \right ) \otimes \disjointgraph_{Z,2^{d-i-2}} \coloneqq \mathcal{G}\).
%     We define a map \(\psi: Y^{\mathcal{S}_{\MP}}_W(1) \to \mathcal{G}\) sending \(A \mapsto (A_1,A_2,\dots,A_{2^i})\) where the \(A_j\)'s are as in \pref{claim:characterizing-link-of-w}. By \pref{claim:characterizing-link-of-w} this map is well defined for every \(A\) and sends link vertices into the vertices of \(\mathcal{G}\). Obviously it is injective, since the direct sum of the \(A_j\)'s is \(A\). Moreover, by the other direction of \pref{claim:characterizing-link-of-w} this is also a bijection, that is, \(\psi^{-1}(A_1,A_2,\dots,A_{2^i})=\sum_{j=1}^{2^i} A_j \in \bar{Y}^{\mathcal{S}_\MP}_{W}(1)\).

%     We prove that \(\psi\) is a graph isomorphism. %Let us start with \(\set{x,y} \in \bar{Y}^{\mathcal{S}_J}_w(2)\) and prove that \(\psi(x)\) and \(\psi(y)\) are neighbors in \(\mathcal{J}\). As \(\set{x,y}\) is an edge, \(y \in \bar{Y}^{\mathcal{S}_J}_{w + \sp(x)}(1)\). Let \(w' = w+ \sp(x)\). 
%     A pair \(\set{A,A'}\) is an edge in \(\bar{Y}^{\mathcal{S}_\MP}_W\) if and only if \(A' \in \bar{Y}^{\mathcal{S}_J}_{W'}(1)\) where \(W'=W+\sp(A)\).
%     Applying \pref{claim:characterizing-link-of-w} to \(W\) and \(A\), we get \(Q_{W'} = \set{A_j} \cup \set{Z_j - A_j}\). Applying \pref{claim:characterizing-link-of-w} to \(W'\) we have that \(A' \in \bar{Y}^{\mathcal{S}_\MP}_{W'}(1)\) if and only if:
%     \begin{enumerate}
%         \item we can decompose \(A'=\sum_{j=1}^{2^{i+1}}A_j'\) such that \(A_{2^{i+1}}'\) is a direct sum with the (direct) sum of vectors in \(Q_{W'}\), and 
%         \item for every \(j < 2^{i+1}\) there is a distinct matrix \(T_j \in Q_{W'}\) such that \(A_j' \subseteq T_j\). Let us re-index the \(A_j'\)'s and \(T_j\)'s with \[T_{j,b} = \begin{cases}
%         A_j & b=0 \\ Z_j - A_j & b=1
%     \end{cases}.\]
%     \end{enumerate}
%     So on the one hand, if \(\psi(A),\psi(A')\) are neighbors, we can take \(A_{j,0}' = GCD(A_j',A_j)\) and \(A_{j,1}' = GCD(A_j',Z_j - A_j)\) which will satisfy the above property (and is well defined by the properties of \(\under^{Z_j}\)). This shows that being an edge in \(\mathcal{G}\) implies being an edge in \(\bar{Y}^{\mathcal{S}_\MP}_W\). For the converse direction, if there exists such a decomposition of \(A'\) then it is straightforward to verify that \(A_j'  =A_{j,0}' + A_{j,1}'\), so \(GCD(A_j',A_j)\) has half the rank of \(A_j'\). In other words, they are edges in the corresponding \(\under^{Z_j}\) and \(\disjointgraph_{Z,2^{d-i-2}}\) graphs. Thus \(\set{\psi(A),\psi(A')} \in \mathcal{G}\).
% \end{proof}


% \section{Draft}
% \input{Yotam's drafts/old/uniqueness_draft}

==> Yotam_s_drafts/old/uniqueness_draft.tex <==
\subsection{Rank based posets}
Up until this point, the admissible functions we used were quite general. However, if we restrict our class of functions we can say quite a lot about the link structure. In particular, we will show for this class a decomposition lemma into a tensor product.

Let \(G \subseteq \F_2^n\) be a set. The rank of a vector \(v\) with respect to \(G\), is the minimal number of elements in \(G\) necessary to write \(v\) as their sum. It is \(\infty\) if \(v \notin \sp (G)\) but henceforth we will assume \(G\) is also a generating set. We say \(G\) is admissible if every \(G' \subseteq G\) such that \(v=\sum_{g \in G'}g\) is a minimal way of writing \(v\) as a sum of elements in \(G\) is independent. We call such sets \(G'\) \emph{minimal}.

For example, if \(G_{\mathcal{J}} = \set{e_1,e_2,\dots,e_n}\) is the standard basis, the rank of an element \(v\) is just its weight. If \(G=\MP(1)\) is the set of rank one matrices inside \(\F_2^{n \times n}\), then the rank of a matrix \(M\) is the usual matrix rank. This second example is also true for the set of rank one tensors in \(\F_2^{n^k}\).

The following notation of a direct sum generalizes the matrix poset direct sum.
\begin{definition}[Abstract direct sum]
    We say that \(w_1+w_2+\dots+w_j\) is a direct sum, and write \(w_1\oplus w_2 \oplus w_j\) if \(\rank(w_1 + w_2 + \dots w_j) = \sum_{\ell=1}^j \rank(w_j)\). We also write \(w_1 \leq w_2\) if \(w_1 \oplus (w_2-w_1)\).
\end{definition}
We observe that as in the matrix domination case, this order \(\leq\) is indeed a partial order. As noted above, when \(G=\MP(1)\) this is the matrix domination poset; in the \(G_{\mathcal{J}}\) case the rank of any vector \(v\) is its weight \(wt(v)\). Hence, \(w_1 \oplus w_2 \oplus \dots  \oplus w_j\) if and only if every pair of distinct vectors is disjoint (as a set).

In this context, an admissible function is \(s:\F_2^d \setminus \set{0} \to \F_2^n\) such that \(\bigoplus_{v \in \F_2^d \setminus \set{0}} s(v)\) is a direct sum. An admissible set of functions \(\mathcal{S}\) is such that all functions \(s \in \mathcal{S}\) are admissible. A \emph{uniform-rank} set of local functions is such that for every \(s_1,s_2 \in \mathcal{S}\) and \(v_1,v_2 \in \F_2^d\) we have \(\rank(s_1(v_1)) = \rank(s_2(v_2))\). We denote this number \(\rank(\mathcal{S})\). %A \emph{permutation invariant} set \(\mathcal{S}\) is such that for every \(s \in \mathcal{S}\) and every permutation \(\pi\) of \(\F_2^d \setminus \set{0}\), \(s(\pi(x)) \in \mathcal{S}\).

If \(\mathcal{S}\) is uniform-rank, then \(Y^{\mathcal{S}}\) is called a \emph{rank-based} induced Grassmann posets.

Both the Johnson Grassmann poset and the Matrix Grassmann posets are rank-based induced Grassmann posets. In the Johnson case \(G\) is the standard basis and in the matrix case \(G\) is the rank \(1\) matrices.

Unfortunately, this is still too general for a meaningful decomposition lemma. For this we also need to define another property of \(G\) which we will call the \emph{direct-meet property}.

\begin{definition}[Meet]
    The \(\Meet\) of a set of elements \(T \subseteq \F_2^n\) is an element \(\Meet(T) \in \F_2^n\) such that for every \(v \in \F_2^n\), if \(v \leq t\) for every \(t \in T\), then \(v \leq \Meet(T)\).     
\end{definition}
We note that a \(\Meet(T)\) does not necessarily exist, but if it exists it is always unique.

\begin{definition}[Direct meet property]
    We say that \(G\) has the \emph{direct-meet property} if for every three elements, \(w_1,w_2,w_3\) such that \(w_1 \oplus w_2 \oplus w_3\), the meet of \(\set{w_1 \oplus w_2,w_1 \oplus w_3}\) exists and is equal to \(w_1\). We say \(\Y^{\mathcal{S}}\) has the direct-meet property if it is a rank based induced complex, where the generating set \(G\) has the direct-meet property.
\end{definition}
Rank based induced complexes \(Y^{\mathcal{S}}\) with the direct meet property are the class of complexes on which we can prove a decomposition lemma.

Let us gain some intuition for the direct-meet by considering some examples. First, let us consider the Johnson case. Let \(G_{\mathcal{J}}=\set{e_1,e_2,\dots,e_n}\) be the standard basis, then the direct-meet property holds. Indeed, the meet of any set \(T\) is the intersection \(\Meet(T) = \bigcap_{t \in T}t\), where we treat the vectors as sets. In particular, the meet of \(w_1 \oplus w_2\) and \(w_1 \oplus w_3\) is \(w_1\). On the other hand, if \(G=\set{e_1,e_2,e_3,e_1+y,e_2+y,e_3+y}\) where \(e_1,e_2,e_3,y\) are independent, then \(G\) does not have the direct-meet property. To see this observe the triple \(w_1=e_1,w_2=e_2,w_3=e_3\) and the vector \(e_1+y\). The triple has a direct sum. However, \(e_1+y \leq w_1+w_2=e_1+e_2=(e_1+y)+(e_2+y)\) and \(e_1+y \leq w_1+w_3=e_1+e_3=(e_1+y)+(e_3+y)\), but \(e_1+y \not \leq e_1 = w_1\).

A more interesting example is the low-rank decomposition case. Let \(G\) be the set of rank \(1\) matrices. Contrary to the Johnson case, there exists a set \(\set{M_1,M_2}\) with no meet. For example let \(e_1,e_2\) be independent, let \(M_1=e_1 \otimes e_1 + e_2 \otimes e_2\) and let \(M_2 = e_1\otimes e_1 + e_2 \otimes (e_1+e_2)\). Both \(A = e_1 \otimes e_1\) and \(B = e_2 \otimes (e_1+e_2)\) are under \(M_1\) and \(M_2\) in the matrix domination order. However, \(A \not \leq B\) and \(B \not \leq A\) and therefore there is no meet to \(\set{M_1,M_2}\). Nevertheless, the rank \(1\) matrices have the direct-meet property:

\begin{claim} \label{claim:direct-meet-matrix-poset}
    The rank one matrices have the direct-meet property.
    %In particular, if for a set of matrices \(T = \set{C_i}_{i \in I}\) there exists a matrix \(B\) such that for every \(i\in I\), \(B \leq C_i\) and \(\row(B) = \bigcap_{i \in I} \row(C_i)\), \(\col(B) = \bigcap_{i \in I} \col(C_i)\). 
    %
    %Then \( \forall i \in I, A \leq C_i\) implies \(A \leq B\).
\end{claim}
This claim essentially abstracts the observation in \cite[Lemma 57]{Golowich2023}. We prove it in the end of this section.

Finally we state an elementary claim about the meet which we will use later on.
\begin{claim} \label{claim:extended-direct-meet-property}
    Let \(G\) have the direct-meet property. Let \(T=\set{w_1,w_2,\dots,w_m}\) be such that \(\bigoplus_{j=1}^m w_j\). Let \(\widehat{T} = \set{v_1,v_2,\dots,v_r}\) be linear combinations of \(T\), i.e.\ \(v_j = \bigoplus_{\ell \in I_j}w_\ell\) for some subsets \(I_j \subseteq [m]\). Then \[\Meet(\widehat{T}) = \bigoplus_{\ell \in \bigcap_{j=1}^r I_j} w_\ell. \qed\]
\end{claim}
The proof is just an induction on the size of \(\widehat{T}\). We omit it.

\subsection{The general decomposition lemma}
Our components for the decomposition lemma are the following.
\begin{definition}[\(z\)-domination graph]
    Let \(z\) be of rank \(4m\). The graph \(\mathcal{T}^{z}\) has vertices
    \[V = \sett{y \leq z}{\rank(y)=2m}.\]
    To sample an edge we sample a random decomposition \(w_1\oplus w_2 \oplus w_3 \oplus w_4 = z\), such that \(\rank(w_i) = m\) and output \(\set{y,y'}\) such that \(y=w_1 \oplus w_2, y'=w_1 \oplus w_3\). The set of edges is the support of this distribution.
\end{definition}

\begin{definition}[\(z\)-link graph]
    Let \(z \in \mathcal{R}(2^d-2^{i})\) and let \(m \leq 2^{i-2}\). The graph \(\mathcal{H}_{z}\) has vertices
    \[V = \sett{y \in \F_2}{\rank(y)=2m, y \oplus z}.\]
    To sample an edge we sample a random vector \(t \geq z\). Then we uniformly sample \(z' \leq t\) such that \(\rank(z') = 4m\) and output an edge in \(\mathcal{T}^{z'}\).
\end{definition}
In order to state our decomposition lemma, we observe the following claim.

\begin{claim} \label{claim:uniqueness-of-image-set-ranks}
    For every \(W \in \Y^{\mathcal{S}}(i)\), and \(s_1,s_2 \in \mathcal{S}_i\) such that \(Im(\widehat{s_1})=Im(\widehat{s_2}) = W\). Then there exists some \(A \in GL_{i}(\F_2)\) such that \(s_2(x) = s_1(Ax)\)\footnote{Note that a priori \(s_1\) and \(s_2\) could have different domains, so technically \(A\) is an isomorphism between the domain of \(s_1\) and that of \(s_2\).}. In particular \(Im(s_1) = Im(s_2)\).
\end{claim}
We will hence denote \(Q_W = \set{z_1,z_2,\dots,z_{2^i-1}}\) to be this image set of a given \(W\). We also denote by \(z_W = \bigoplus_{j=1}^{2^i-1}z_j\).

This claim is a consequence of the direct-meet condition. We prove it below and for now, let us proceed to the decomposition lemma and overview its proof.

\begin{lemma}\label{lem:generalized-decomposition-lemma}
    Let \(W \in \Y^{\mathcal{S}}(i)\) with \(Q_W = \set{z_j}_{j=1}^{2^i - 1}\) as above and let \(z = \bigoplus_{j=1}^{2^i} z_j\). Then \(\Y_W \cong \mathcal{T}^{z_1} \otimes \mathcal{T}^{z_2} \otimes \dots \otimes \mathcal{T}^{z_{2^i-1}} \otimes \mathcal{H}_{z_W}\).
\end{lemma}
We observe that this lemma for \(\Y^{\mathcal{S}_{\mathcal{J}}}\) is \pref{lem:links-of-Johnson}. For \(\Y^{\mathcal{S}_{\MP}}\) this is \pref{lem:grassmannian-link-decomposition}. We can even generalize this lemma slightly more to capture the sparsified matrix case. See \pref{sec:distribution-over-admissibles} for the details.

The proof of \pref{lem:generalized-decomposition-lemma} uses the following argument. First we give a combinatorial criterion for a vector \(y \in \Y_W^{\mathcal{S}}(1)\), in terms of its meets with the elements in \(Q_W\). 

\begin{claim} \label{claim:abstract-unique-decomposition}
    Let \(W \in \Y^{\mathcal{S}}(i)\) with \(Q_W = \set{z_1,z_2,\dots,z_{2^i-1}}\) as above. Let \(y \in \F_2^n\). Then \(y\) is in the link of \(W\) if and only if there exists \(y_1,y_2,\dots,y_{2^i}\) with the following properties:
    \begin{enumerate}
        \item \(y = \bigoplus_{j=1}^{2^i} y_j\) (that is, \(y\) is equal to the sum of all \(y_j\)'s and this sum is direct).
        \item All \(y_j\)'s have equal rank.
        \item \(y_i \leq z_i\).
    \end{enumerate}
    In this case with \(W' = W + \sp(y)\), we have \(Q_{W'} = \set{z_j}_{j=1}^{2^i-1} \cup \set{z_j - y_j}\).
\end{claim}

Given this claim, we can define the isomorphism \(\psi: \Y_W \to \mathcal{T}^{z_1} \otimes \mathcal{T}^{z_2} \otimes \dots \otimes \mathcal{T}^{z_{2^i-1}} \otimes \mathcal{H}_{z_W}\) by \begin{equation}\label{eq:iso-for-decomp-lemma}
\psi(y)=(y_1,y_2,\dots,y_{2^i}),
\end{equation}
where the image are the unique \(y_j\)'s given in \pref{claim:abstract-unique-decomposition}. This function is also a bijection by \pref{claim:abstract-unique-decomposition}.

To conclude the proof, we need to argue that an edge \(\set{y,y'}\) is sampled by sampling the different components \(y_j,y_j'\) independently from one another. For this part, we basically need the fact that conditioned on part of the values of \(s\) on \(R \subseteq \F_2^d\), the rest of the values of \(s(v)\) for \(v \notin R\), depend only on the sum, \(\sum_{v \in R}s(v)\), and not on the values themselves.
\begin{claim} \label{claim:independence-given-sums}
    Let \(\mathcal{S}\) be a rank-based poset. Let \(R_1,R_2,\dots,R_m \subseteq \F_2^d \setminus \set{0}\) be a partition.  Let \(z_1,z_2,\dots,z_{m-1} \in \F_2^d\) be such that \(\rank(z_i) = |R_i|\cdot r\) and such that there exists some \(s \in \mathcal{S}\) with \[z_1 \oplus z_2 \oplus \dots \oplus z_{m-1} \leq \bigoplus_{v \in \F_2^d \setminus \set{0}} s(v).\]

    Let \(\set{P_i = s|_{R_i}}_{i=1}^m\) be joint random variables and let \(\set{Q_i}_{i=1}^m\) be the random variables \(\set{P_i}_{i=1}^m\) conditioned on the event that for every \(i=1,2,\dots,m-1\)
    \[\sum_{v \in R_i} s(v)=z_i.\]
    Then \(\set{Q_i}_{i=1}^m\) are independent.
\end{claim}

% To conclude the proof we will show that \(\set{y,y'}\) are an edge in \(\Y_W\) if and only if their \(\psi\)-images are an edge in the tensor product. Here the argument follows again from \pref{claim:abstract-unique-decomposition} and some definition chasing, but this time \pref{claim:abstract-unique-decomposition} is applied to the \(i+1\)-dimensional space \(W' = W \oplus \sp (y)\). The proof itself is slightly more subtle, because technically the edges in are also weighted, so we need to argue that the weight of an edge in \(Y_W\) is the product of the weights of the corresponding edges in \(\mathcal{T}^{z_1} \otimes \mathcal{T}^{z_2} \otimes \dots \otimes \mathcal{T}^{z_{2^i-1}} \otimes \mathcal{H}_{z_W}\). However, this is just a calculation.

\begin{proof}[Proof of \pref{lem:generalized-decomposition-lemma}]
    Let us denote by \(\mathcal{G} = \mathcal{T}^{z_1} \otimes \mathcal{T}^{z_2} \otimes \dots \otimes \mathcal{T}^{z_{2^i-1}} \otimes \mathcal{H}_{z}\).
    We define a map \(\psi: Y^{\mathcal{S}}_W(1) \to \mathcal{G}\) sending \(y \mapsto (y_1,y_2,\dots,y_{2^i})\) as in \eqref{eq:iso-for-decomp-lemma}. That is, the \(y_j\)'s are as in \pref{claim:abstract-unique-decomposition}. By \pref{claim:abstract-unique-decomposition}, this map is well defined for every \(y\) and sends link vertices into the vertices of \(\mathcal{G}\). Moreover, by \pref{claim:abstract-unique-decomposition} this is also a bijection, since the map \[\psi^{-1}(y_1,y_2,\dots,y_{2^i}) \coloneqq \bigoplus_{j=1}^{2^i} y_j \in \bar{Y}^{\mathcal{S}}_{W}(1)\]
    is its inverse according to the claim.

    Let us now prove that a pair \(\set{y,y'}\) is an edge in \(\bar{Y}^{\mathcal{S}}_W\) if and only if \(\set{\psi(y),\psi(y')}\) is an edge in \(\mathcal{G}\). Recall that \(\set{y,y'}\) is an edge in \(\bar{Y}^{\mathcal{S}}_W\) if and only if \(y' \in \bar{Y}^{\mathcal{S}_J}_{W'}(1)\) where \(W'=W+\sp(y)\).
    By \pref{claim:abstract-unique-decomposition}, \(Q_{W'} = \set{y_j}_{j=1}^{2^i} \cup \set{z_j - y_j}_{j=1}^{2^i-1}\). 
    Let us re-index \(t_j \in Q_{W'}\)'s with \[t_{j,b} = \begin{cases}
            y_j & b=0 \\ z_j - y_j & b=1
    \end{cases}.\]
    for \((j,b) \in [2^i - 1] \times \set{0,1} \cup \set{(2^i,0)}\). 
    Moreover, by applying \pref{claim:abstract-unique-decomposition} to \(W'\) we have that \(y' \in \bar{Y}^{\mathcal{S}}_{W'}(1)\) if and only if:
    \begin{enumerate}
        \item We can decompose \(y'=\bigoplus_{(j,b)\in [2^i] \times \set{0,1} }y_{j,b}\) such that where the rank of every summand is equal and 
        \item For every \((j,b) \ne (2^i,1)\) there is a distinct vector \(y_{j,b} \leq t_j\).
        \item The final \(y_{2^i,1}\) is a direct sum with \(z_{W'}\) (the sum of all elements in \(Q_{W'}\)).
    \end{enumerate}

    So on the one hand, if \(\psi(y),\psi(y')\) are neighbors, we can take \(y_{j,0}' = \Meet(y_j',y_j)\) and \(y_{j,1}' = \Meet(y_j',z_j - y_j)\) which will satisfy the above property (and is well defined by the properties of \(\under^{z_j}\)). This shows that being an edge in \(\mathcal{G}\) implies being an edge in \(\bar{Y}^{\mathcal{S}}_W\). For the converse direction, suppose there exists such a decomposition of \(y'\). Then for every \(z_j\) the vectors, \(w_1 = y_{j,0}', w_2=y_{j,1}', w_3 = t_{j,0}-y_{j,0}'\) and \(w_4 = t_{j,1}-y_{j,1}'\) have that \(w_1\oplus w_2 = y_j'\) and \(w_1\oplus w_3 = y_j\). \Ynote{Technically we need to add some purity assumption:} In addition they are equal rank. Thus concluding that \(\set{y_j,y_j'}\) are an edge in \(\mathcal{T}^{z_j}\). For the final component, a similar calculation holds: we take an element containing \(z'\) that is a direct sum with \( z_{W'}\oplus y_{2^{i+1}}\) and such that \(\rank(z') = 4\rank(y_{2^i,1})\). We decompose it into \(w_1 = y'_{2^i,0}\), \(w_2 = y_{2^i}-y'_{2^i,0}\), \(w_3 = y'_{2^i,1}\) and \(w_4 = z'-w_1-w_2-w_3\). These \(w_i\)'s show that \(\set{y_{2^i},y_{2^i}'}\) are an edge in \(\mathcal{H}_{z_W}\). the components \(y_{2^i}\). Thus \(\set{\psi(y),\psi(y')} \in \mathcal{G}\).

    Finally, we note that sampling every \(\set{y_j,y_j'}\) in an edge is done independently. Indeed, conditioned on sampling \(W\) in a link is the same as conditioning that for some \(d-i\)-dimensional subspace \(V_0\), the values \(s_{V_0}(v+V_0)\) are fixed. For every \(j \leq 2^i - 1\), there exists some \(v+V_0\) such that \(\set{y_j,y_j'}\) depend only on the values of \(v' \in V_0\) (this is the \(v+V_0\) such that \(y_j,y_j' \subseteq s_{V_0}(v+V_0)\). For the final component \(\set{y_{2^i},y_{2^i}'}\), this edge only depends on the values of \(s\) on \(0+V_0\). By \pref{claim:independence-given-sums}, the values of \(s\) on the respective parts in each coset \(v+V_0\) are independent once all values of \(s_{V_0}\) have been fixed. We conclude that indeed \(\psi\) is an isomorphism.
    
    % Finally, we need to show that the probability of sampling an edge \(\set{y,y'}\) is the product of probabilities of sampling \(\set{y_j,y_j'}\) in the components of the tensor product.
    
    % Let us describe the probabilistic experiment that samples an edge in the link in a way that is convenient to us. To sample an edge in the link we first sample \(W'' \in \Y_W(i+2)\) and then uniformly sample \(y,y'\) such that \(W'' = W \oplus \sp(y,y')\). Thus we claim that for every \(W_0\in \Y_W(i+2)\)
    % \begin{equation} \label{eq:prob-sampling-link-edge}
    %     \Prob[W'' \sim \Y_W(2)]{W''=W_0} = \cProb{s \sim \mathcal{S}}{Im(\widehat{s_{V_2}}) = Q_{W_0})}{Im(\widehat{s_{V_0}}) = Q_{W}},
    % \end{equation}
    % where \(V_0 \supseteq V_2\) are two arbitrary \emph{fixed} subspaces of \(\F_2^d\) of dimensions \(\dim (V_0) = d-i\) and \(\dim (V_2) = d-i-2\).

    % Let us explain why \eqref{eq:prob-sampling-link-edge} holds. To sample a pair of \(i\) and \(i+2\) subspaces \((W,W'')\) we first sample a function \(s \in \mathcal{S}\), which gives \(Im(\widehat{s}) \in \Y(d)\). Then we sample some \(W \subseteq W'' \subseteq Im(\widehat{s})\) of dimension \(i\) and \(i+2\) uniformly at random. This second step is equivalent to sampling \(U \subseteq U'' \subseteq \F_2^d\) of dimension \(i\) and \(i+2\) uniformly at random, and outputting \(W = Im(\widehat{s}|_U), W'' = Im(\widehat{s}|_U)\).
    
    %  However, if \(\mathcal{Y}^{\mathcal{S}}\) is rank-based, we observe that if \(s \in \mathcal{S}\) then for every \(A \in GL_{d}(\F_2)\) the function \(s(Ax) \in \mathcal{S}\) as well. Therefore, we can just \emph{fix} an arbitrary \(i\) and \(i+2\) dimensional subspaces \(U_0 \subseteq U_2 \subseteq \F_2^d\) and sample \(W,W''\) by just sampling \(s \in \mathcal{S}\) uniformly at random and outputting \(W = Im(\widehat{s}|_{U_0})\), \(W'' = Im(\widehat{s}|_{U_2})\). Now, with \(V_0 = U_0^\bot\) and \(V_2 = U_2^\bot\), it is equivalent to output \(W=Im(\widehat{s_{V_0}})\) and \(W''=Im(\widehat{s_{V_2}})\) by \pref{claim:skeleton-of-induced-Grassmann}. By \pref{claim:uniqueness-of-image-set-ranks}, \(W=Im(\widehat{s_{V_0}})\) if and only if \(Im(s_{V_0}) = Q_W\) and similarly for \(W''\). Thus, sampling \(W''\) conditioned on \(W\) is the same as sampling \(s \in \mathcal{S}\) such that \(Im(s_{V_2}) = Q_{W''}\) conditioned on \(Im(\widehat{s_{V_0}}) = Q_{W}\). Thus \eqref{eq:prob-sampling-link-edge} holds.

    % Fix a function \(s_{V_0}\) whose image is \(Q_W\). For every \(z \in Q_W\) there are exactly four \(z'_1,z'_2,z'_3,z'_4 \in Q_{W''}\) such that \(z'_i \leq z\); these have that \(z'_1 \oplus z'_2 \oplus z'_3 \oplus z'_4 = z\); the rest of the \(z' \in Q_{W''}\) are a direct sum with \(z\). Let \(v+V_0 \ne 0 + V_0\) and suppose that it decomposes to \(v+v_0 = t_1+V_2 \dunion t_2+V_2 \dunion t_3+V_2 \dunion t_4+V_2\). Conditioning that \(s_{V_0}(v+V_0) = z\) is just conditioning that \(\sum_{j=1}^4 s_{V_2}(t_j+V_2) = z\). Finally, we note that there are three elements in \(Q_{W''}\) that are a direct sum with \(z_W\). These are the elements that are supposed to be the images of the three equivalence classes of \(0+V_0 \setminus 0+V_2\).
    
    % Hence, choosing some \(s_{V_2} \in \mathcal{S}_{i+2}\) such that \(Im(s_{V_2}) = Q_{W''}\) conditioned on \(Im(s_{V_0}) = Q_W\) is done by \emph{independently} choosing a decomposition of every \(z_j \in Q_W\) to four components of equal rank uniformly at random and independently, and also choosing three \(z_1,z_2,z_3\) that are a direct sum with \(z_W\) (also independent of the rest of the choices).

    % Finally, we note that \(x,x'\) such that \(U \oplus \sp(x,x') = U_2\) has the property that out of every four \(t_1+V_2, t_2+V_2, t_3+V_2, t_4 + V_2\) that comprise some \(v+V_0\), there is exactly 
\end{proof}

We conclude this subsection with the proofs of \pref{claim:uniqueness-of-image-set-ranks}, \pref{claim:independence-given-sums} and \pref{claim:abstract-unique-decomposition}.
\begin{proof}[Proof of \pref{claim:uniqueness-of-image-set-ranks}]
    Let \(s\) be such that \(Im(s)=W\) such that the domain of \(s\) is \(U \setminus \set{0}\). Observe that by \pref{claim:extended-direct-meet-property}, \(s(x) = \Meet(\sett{\widehat{s}(y)}{y \in U, \iprod{x,y}=1})\), since \(s(x)\) the subset of the right are linear combinations of a bunch of \(s(x')\) which are a direct sum, and \(s(x)\) is the only common part in the linear sums of \(\widehat{s}(y)\).

    Now assume that \(Im(\widehat{s_2}) = Im(\widehat{s_1})\). This implies that there is an isomorphism \(B\) such that \(\widehat{s_1}(x)=\widehat{s_2}(Bx)\). On the other hand, by the above
    \begin{align*}
        s_1(x) &= \Meet(\sett{\widehat{s_1}(y)}{y \in U, \iprod{x,y}=1})\\
        &=\Meet(\sett{\widehat{s_2}(By)}{y \in U, \iprod{x,y}=1})\\
        &=\Meet(\sett{\widehat{s_2}(By)}{By \in U, \iprod{x,B^{-1} By}=1})\\
        &\overset{y'=By}{=}\Meet(\sett{\widehat{s_2}(y')}{y' \in U, \iprod{x,B^{-1} y'}=1})\\
        &=\Meet(\sett{\widehat{s_2}(y')}{y' \in U, \iprod{(B^{-1})^T x,y'}=1})\\
        &= s_2((B^{-1})^T x).
    \end{align*}
    Set \(A = (B^{-1})^T\) and we got \(s_1(x)=s_2(Ax)\).
    % Let us explain why. Every \((i-1)\)-dimensional subspace of \(U\) is given by \(\sp(v)^{\bot} \cap U\) for some \(v+V \in \nicefrac{\F_2^d}{V} \setminus \set{0+V}\) (and \(\sp(v)^{\bot} \cap U = \sp(v')^{\bot} \cap U\) if and only if \(v+V = v'+V\)). Thus the set \(\sett{s_V(v+V)}{v+V \ne V}\) is equal to 
    % \[ \sett{\Meet(\sett{\widehat{s_V}(x)}{x \in U \setminus U'}) }{U' \subseteq U, \dim(U')=i-1}.\]
    % Writing \(W = Im(\widehat{s_V}) = Im(\widehat{s_{V'}})\) this is also equal to 
    % \[ \sett{\Meet(W \setminus W')}{W' \subseteq W, \dim(W')=i-1}\]
    % since going over all \(U' \subseteq U\) of dimension \((i-1)\) in the domain is the same as going over all subspaces inside the image, is the same as going over all subspaces of \(W\) of the same dimension. As we can see, this set is independent of \(s_V\) since it has a description depending only on vectors and subspaces of \(W\).
\end{proof}

\begin{proof}[Proof of \pref{claim:abstract-unique-decomposition}]
    Let \(s \in \mathcal{S}\) and \(U' \subseteq \F_2^{d}\) be such that \(Im(\widehat{s}|_{U'}) = W'\) and let \(U \subseteq U'\) be such that \(Im(\widehat{s}|_{U}) = W\). Write \(V = \sp \set{b_1,b_2,\dots,b_{d-i}}\) and \(V' = \sp \set{b_1,b_2,\dots,b_{d-i-1}}\) such that \(U'=V'^{\bot}\) and \(U=V^\bot\). We recall that every \(v+V \in \nicefrac{\F_2^d}{V}\) can be partitioned into two cosets of \(V'\), \(v+V = v+V' \dunion (v+b_{d-i})+V'\) and therefore \(s_V(v+V) = s_{V'}(v+V') + s_{V'}((v+b_{d-i})+V')\). By the fact that \(s_{V'} \in \mathcal{S}_i\) this sum is also direct.
    
    Let \(x \in U' \setminus U\) be such that \(\widehat{s}(x)=y\). By \pref{claim:skeleton-of-induced-Grassmann}, it also holds that \(\widehat{s_{V'}}(x)=A\). By the fact that \(x \in U' \setminus U\), the inner product \(\iprod{x,b_{d-i}} = 1\) and therefore, \(\iprod{x,v+V'} \ne \iprod{x,(v+b_{d-i})+V'}\). This implies that that for every \(v_0+V \ne V\), exactly one of \(y_j \in \set{s_{V'}(v_0+V'), s_{V'}((v_0+b_{d-i})+V')}\) has \(y_j \leq y\). Indeed:
    \begin{align*}
        y = \widehat{s_{V'}}(x) &= \sum_{v+V' \not\subseteq 0+V} \iprod{x,v+V'}s_{V'}(v+V') \\
    &+  \iprod{x,v_0+V'}s_{V'}(v_0+V') \\
    &+ \iprod{x,(v_0+b_{d-i})+V'}s_{V'}(v_0+b_{d-i}+V').
    \end{align*}
Assume that \(\iprod{x,v_0+V'}=1\) and thus \(\iprod{x,(v_0+b_{d-i})+V'} = 0\) (the other case is similar). In this case because this whole sum is actually disjoint then every non-zero component in the sum has is \(\leq y\). In particular \(s_{V'}(v_0+V') \leq y\). Moreover, any component that does not appear in this sum is a direct sum with \(y\), and in particular \(s_{V'}(v_0+b_{d-i}+V') \not \leq y\).

Thus we re-index \(z_j = s_V(v+V)\) (arbitrarily) and set \(y_j\) to be the component where \(y_j \leq y\) and \(y_j \leq s_V(v+V)\). We also set \(y_{2^i} = s_{V'}(b_{d-i})\) and note that \(y_{2^i}\) also participates in the linear combination of \(\widehat{s_{V'}}(x)\) because \(\iprod{x,b_{d-i}}=1\). All \(y_j\)'s have rank \(2^{d-i-1}\) and by the discussion above, we have that \(y = \sum_{j=1}^{2^i} y_j\). Moreover, \(y_j \leq y_j\) for every \(j \leq 2^i-1\) and \(y_{2^i}\) is a direct sum with the sum of \(z_j = s_V(v+V)\). Thus, \(Q_{W'} = \sett{s_{V'}(v+V')}{v+V' \ne V'} = \set{y_j}_{j=1}^{2^i} \cup \set{z_j-y_j}_{j=1}^{2^i - 1}\) by construction. Finally, we note that the when the admissible functions come fro ma rank-based construction that has the direct-meet property, \(y_j = \Meet(y,s_{V}(v_0+V)\) for one of the \(v_0 + V\). Thus, the \(y_j\)'s are unique.

\medskip

Conversely, let us assume that the three items hold and prove that \(W' \in \Y(i+1)\). Let \(s \in \mathcal{S}_i\) be such that \(Im(\widehat{s})=W\). Recall that \(\mathcal{S}_{i+1}\) are all functions \(s'\) whose image contains vectors of rank \(2^{d-i}\) whose sum is direct. Therefore, let us construct such a function \(s':\F_2^{i+1} \to \F_2^n\) where \(Im(\widehat{s})=W'\). First, we re-index the elements \(y_j\) as \(y_v\)'s for every \(v \in \F_2^{i} \setminus \set{0}\), such that \(y_v \leq s(v)\) (but keep the notation \(y_{2^i}\) as before). For an input \((b,v)\in \F_2 \times \F_2^{i} \setminus \set{\bar{0}}\),
    \[s'(b,v) = \begin{cases} y_v + (1-b)s(v) & v \ne 0 \\ y_{2^i} & (b,v)=(1,\bar{0}) \end{cases}.\]
It is easy to see that the image of \(s'\) is \(\set{y_j}_{j=1}^{2^i} \cup \set{z_j - y_j}_{j=1}^{2^i - 1}\) which is a direct sum of vectors of rank \(2^{d-i-1}\), thus \(s' \in \mathcal{S}_{i+1}\). Moreover, one readily verifies that \(\widehat{s'}(1,\bar{0}) = \sum_{v \in \F_2^i} s'(1,v) = \sum_{j=1}^{2^i} y_j = y\) and that for \(U'' = \sett{(0,v)}{v \in \F_2^i}\) we have that \(Im(\widehat{s'}|_{U''}) = W\). Thus \(Im(\widehat{s'}) = W'\).
\end{proof}


\begin{proof}[Proof of \pref{claim:independence-given-sums}]
    It suffices to show that \(Q_i\) is independent of \(Q_{[m] \setminus \set{i}}\) where \(Q_{[m] \setminus \set{i}}\) denotes the rest of the random variables. For \(i < m\) and \(s_0:R_i \to \F_2^d\), the probability that \(P_i = s_0\) is uniform among all \(s_0\) such that \(\rank(s_0(v))=r\) and \(\bigoplus_{v \in R_i}s_0(v_i) = z_i\). This just follows from the fact that conditioning on the values of \(s|_{(\F_2^d \setminus \set{0}) \setminus R_i}\) (in addition to the conditioning of \(z_i\)), all such functions \(s_0\) are equally likely.

    For \(i=m\), as similar argument holds. Conditioned on any specific values of \(s|_{R_1},s|_{R_2},\dots,s|_{R_{m-1}}\) (that sum up to the respective \(z_i\)'s), the choice of \(s|_{R_m}\) is a uniform (ordered) choice of the elements \(t_1,t_2,\dots,t_{|R_m|}\) of rank \(r\) such that \(\left (\bigoplus_{j=1}^{m-1} z_j \right ) \oplus \left ( \bigoplus_{j=1}^{|R_m|} t_j \right )\). It is obvious that this independent of the specific values assigned to \(s|_{R_1},s|_{R_2},\dots,s|_{R_{m-1}}\).
\end{proof}

\subsection{The distribution over admissible functions} \label{sec:distribution-over-admissibles}
We can extend the decomposition lemma above, to a slightly more general setup where instead of sampling \(s \in \mathcal{S}\) uniformly, we sample it according to a measure. Let \(\mathcal{S}\) be a uniform-rank set of admissible functions. Let \(\mu\) be a probability density over \(\mathcal{S}\). We say that \(\mu\) is permutation invariant if for every \(s \in \mathcal{S}\) and every permutation \(\pi\) of \(\F_2^d \setminus \set{0}\),  \(\mu(s)=\mu(s \circ \pi)\). Such a measure induces a measure on \(\Y^{\mathcal{S}}(d)\) be the rank-based induced poset obtained, equipped with the probability density over \(d\)-subspaces where one samples \(s \sim \mu\) and then outputs \(Im(\widehat{s})\). We call posets obtained by this process \emph{measured rank-based posets}. This generalizes the case discussed above where \(\mu\) is uniform.

We note that the sparsified matrix poset is a measured rank-based posets, where the measure \(\mu(s)\) is the probability of sampling \(s\) by the following process: sample \(W_1, W_2 \in \Y_0(2^d -1)\) independently and sample \(s\) uniformly at random such that \(\row(\bigoplus_{v \in \F_2^d \setminus \set{0}} s(v)) = W_1\) and \(\col(\bigoplus_{v \in \F_2^d \setminus \set{0}} s(v)) = W_2\). This poset it is not necessarily an (unmeasured) rank-based poset so this more generalized definition captures this example as well.

For such posets we can prove a version of the decomposition lemma with the following graph variant.
\begin{definition}[\((z,\mu)\)-link graph]
    Let \(z \in \mathcal{R}(2^d-2^{i})\) and let \(m \leq 2^{i-2}\). The graph \(\mathcal{H}^\mu_{z}\) has vertices
    \[V = \sett{y \in \F_2}{\rank(y)=2m, y \oplus z}.\]
    To sample an edge we sample a random vector \(s \sim \mu\) conditioned on \(t \geq z\) where \(t=\bigoplus_{v \in \F_2^d \setminus \set{0}}s(v)\). Then we uniformly sample \(z' \leq t\) such that \(\rank(z') = 4m\) and output an edge in \(\mathcal{T}^{z'}\).
\end{definition}

\begin{lemma}
  Let \(\Y^{\mathcal{S}}\) be a measured rank-based poset with the direct-meet property. Then for every \(W \in \Y^{\mathcal{S}}(i)\) with \(Q_W = \set{z_1,z_2,\dots,z_{2^i-1}}\) and \(z= \sum_{j=1}^{2^i-1} z_j\),
  \[\Y^{\mathcal{S}}_W \cong \mathcal{T}^{z_1} \otimes \mathcal{T}^{z_2} \otimes \dots \otimes \mathcal{T}^{z_{2^i-1}} \otimes \mathcal{H}^{\mu}_{z}.\]
\end{lemma}
The proof of this lemma is follows the exact same proof of the decomposition lemma \Ynote{Cite}. Therefore we omit the proof for brevity.

\subsection{The matrices have the direct-meet property}
\begin{proof}[Proof of \pref{claim:direct-meet-matrix-poset}]
    The technical statement we prove is the following: Let \(A,B \leq C\) be such that \(\row(A) \subseteq \row(B)\) and \(\col(A) \subseteq \col(B)\). Then \(A \leq B\).

    Let us first show that this statement implies the direct meet property. Let \(M_1,M_2,M_3\) be three matrices whose sum is direct. We observe that \(\row(M_1) = \row(M_1 \oplus M_2) \cap \row(M_1 \oplus M_3)\) and similarly for the column space (it is clear that \(\row(M_1) \subseteq  \row(M_1 \oplus M_2) \cap \row(M_1 \oplus M_3)\). The other direction follows from a dimension count). Let \(A \leq M_1 \oplus M_2\) and \(A \leq M_1 \oplus M_3\). We show that \(A \leq M_1\). Observe that \(\row(A) \leq \row(M_1 \oplus M_2) \cap \row(M_1 \oplus M_3)\). Thus \(\row(A) \subseteq \row(M_1)\). This is of course also true for the respective column spaces, and so \(A \leq M_1\).

    Now for the statement itself. Observe that \(\row(B-A) \subseteq \row(B)\) and \(\col(B-A) \subseteq \col(B)\). Moreover, \((C-B) \oplus B\) which means that \(\row(C-B)\) and \(\col(C-B)\) intersects trivially with \(\row(B)\) and \(\col(B)\) respectively. Thus \((C-B) \oplus (B-A)\). So we get
    \[ \rank(C-A) = \rank((C-B) + (B-A)) = \rank(C-B) + \rank(B-A).\]
    On the other hand, because \(A,B \leq C\) this translates to
    \[\rank(C) - \rank(A) = \rank(C) - \rank(B) + \rank(B-A)\]
    or equivalently \(\rank(B) = \rank(A) + \rank(B-A)\) i.e.\ \(A \leq B\).
\end{proof}



% The following distribution is a natural distribution over admissible functions, that can be seen as a generalization of the distribution over simplicial complexes. Although this may seem like an unnecessary complication at first, making use of this distribution will simplify the analysis of our decomposition lemma below, and will also help us capture some additional examples of interesting posets.

% Denote \(\mathcal{R}(j)\) be the vectors of rank \(j\). Given a probability density \(\mu:\mathcal{R}(2^d) \to [0,1]\) we define the following distribution over admissible functions by the following process.
% \begin{enumerate}
%     \item Sample \(v \sim \mu\).
%     \item Uniformly sample \(s_0,s_1 \in \mathcal{R}(2^{d-1})\) such that \(s_0 \oplus s_1 = v\).
%     \item For \(i=2,\dots,d\) define the following vectors \(\set{s_x}_{x \in \F_2^i}\) iteratively, where at the \(i\)-th step the vectors \(s_{x0},s_{x1} \in \mathcal{R}(2^{d-i})\) are sampled such that \(s_x = s_{x0} \oplus s_{x1}\).
%     \item Uniformly sample \(G \in GL_{d}(\F_2)\).\footnote{This step is not necessary and does not affect the outcome complex \(\Y^{\mathcal{S}}\). However, we will see later that this step makes this distribution to be easier to analyze.}
%     \item Output \(s:\F_2^d \to \set{0}\) given by \(s(x)=s_{Gx}\).
% \end{enumerate}

% A natural choice for \(\mu\) is just the uniform distribution. This is the distribution of choice when considering the Johnson poset or the matrix poset.

% However, using such a distribution, allows us to also capture the other example in the section, the \emph{sparsified} matrix poset. In this example, we use the same set \(G = \MP(1)\) of rank one matrices, but the measure \(\mu\) samples a rank \(2^d\) matrix by first sampling a pair of subspaces \(W_1,W_2 \in \Y_0(2^d)\), and then sample a matrix \(M\) conditioned on \(\row(M) = W_1, \col(M) = W_2\). This is the generality necessary to capture all our examples.

==> Yotam_s_drafts/old/upp-matrix-lemma.tex <==


Let us define a bipartite version of \(G_{M,a,0}\). 

It turns out that this graph is 
\begin{corollary}
    Let \(i,j \leq m\) such that \(i+j+2 \leq m\). Let \(H^m_{i,j}\) be the bipartite graph defined by
    \[L = \sett{A \leq M}{\rank(A) = i}\]
    \[R = \sett{A \leq M}{\rank(A) = j}\]
    and 
    \(E \sett{(A,A')}{A \leq A'}\). Then there exists some constant \(\eta > 0\) so that \(\lambda(H^m_{i,j}) \leq 2^{-c(j-i)}\) independent of \(i,j\) and \(m\).
\end{corollary}

==> Yotam_s_drafts/recursive_louis_intro.tex <==
\subsection*{draft}


\subsection*{Draft Overview}
Let us start with an overview of the Golowich's construction \cite{Golowich2023}. The main component in this construction is a sparsification of a different kind of high dimensional structure - the Grassmann poset. The Grassmann poset \(\Gr\), is the poset of all subspaces of \(\F_2^n\) ordered by containment, and a sparsification of \(\Gr\) is a sub-poset \(\Y \subseteq \Gr\) that is downward closed to containment\footnote{I.e.\ if \(w_1 \subseteq w_2\) and \(w_2\) is in the poset, then \(w_1\) is also in the poset.}. We denote by \(\Y(i)\) the \(i\)-dimensional subspaces of \(\Y\) and we say that \(\Y\) is \(d\)-dimensional if a maximal subspace in \(Y\) has dimension \(d\).

The two properties that are important to us in \(\Y\) is its expansion and size. The expansion refers to the spectral expansion of the graph \(G_\Y=(V,E)\) whose vertices are \(V=\Y(1)\) and a pair of subspaces \(\set{w_1,w_2} \in E\) if \(w_1 + w_2 \in \Y(2)\). %We say that \(\Y\) is a  \([\diml,n,\degree,\lambda]\)-poset if \(\Y\) is a \(\diml\)-dimensional poset of \(\F_2^n\) where \(\abs{\Y(1)} \leq 2^\degree\) and such that \(G_\Y\) is a \(\lambda\)-spectral expander.

\cite{Golowich2023} gives a blackbox transformation going from a sparsification \(\Y\) of the Grassmann poset with \(|\Y(1)|=K\) to a Cayley HDX over \(\F_2^n\) with \(K\) generators, which they call `the basification complex', provided that the subspaces in \(\Y(1)\) span \(\F_2^n\). Therefore we focus on the question of sparsifying the Grassmann poset.

Let \(n=k^2\). The sparsified Grassmann poset \(\M_{Gol}\) in \cite{Golowich2023} identifies \(\F_2^n\) with \(\F_2^{k \times k}\), the space of \(k \times k\) matrices. Golowich constructs a poset whose \(1\)-dimensional subspaces are (the spans of) all \(r\)-rank matrices, for a fixed constant \(r\) (we will abuse notation and write \(M \in \M_{Gol}(1)\) instead of \(\sp(M) \in \M_{Gol}(1)\)). Already we note that in this case \(\abs{\M_{Gol}(1)} = 2^{O_r(k)}=2^{O_r(\sqrt{n})}\) which corresponds to the subpolynomial degree of the complex in \cite{Golowich2023}.

The span \(\sp(M_1,M_2)\) is in the sparsified Grassmann if we can decompose \(M_1 = B+C_1\) and \(M_2 = B+C_2\) where \(B,C_1\) and \(C_2\) have rank \(\frac{r}{2}\), and the row and column spans of \(C_1\) and \(C_2\) intersect trivially. Note that in this case \(M_1+M_2\) also has rank \(r\), and so this poset is indeed downward closed to containment. The expansion in this case is a simple argument since this graph is almost the complete graph, although we comment that the analysis of higher dimensional version is much more subtle.

Our construction is an iterative version of \(\M_{Gol}\). Our sparsification takes a \(\frac{3}{2}r\)-dimensional sub-poset \(\Y\) as a parameter so we denote it by \(\M(\Y)\) (but just use \(\M\) for short when \(\Y\) is clear). Its \(1\)-dimensional subspaces are all \(r\)-rank matrices \emph{whose row and column spaces are in \(\Y(r)\)}. A two dimensional subspace \(\sp(M_1,M_2) \in \M\) if it is in \(\M_{Gol}\) and if \(\row(M_1) \oplus \row(M_2)\) and \(\col(M_1) \oplus \col(M_2)\) are in \(\Y(\frac{3r}{2})\) (here \(\row(M),\col(M)\) is notation for the row and column spaces). Namely, given a sparsification \(\Y\) for the \(\F_2^k\)-Grassmann, we obtain a sparsification \(\M(\Y)\) for the \(\F_2^{k \times k}\)-Grassmann, with \(\abs{\M(1)} = O(\abs{\Y(r)})\). Now we can reiterate this construction and obtain a sequence of posets that become sparser and sparser: \(Y_0,\Y_1,\dots\) where \(Y_0 = \Gr\) is \(Y_{i+1} = \M(Y_i)\). Here \(\Y_m\) is a sub-poset of the \(\F_2^{k^{2^m}}\) Grassmann, but with \(\abs{\Y_m (0)} = 2^{O_m(k)}\).

Our main proposition is that whenever \(\Y\) is sufficiently expanding and has sufficiently high dimension, then \(\M(\Y)\) expands as well. We won't describe the complete analysis since it is delicate, and also applies a lot of the machinery developed in \cite{Golowich2023}. We will say that one main tool is 

There are also other technical differences between our version of the Grassmann of the one in \cite{Golowich2023}, which mean that we need to 
